The preparation of states in quantum mechanics

The important problem of how to prepare a quantum mechanical system, $S$, in a specific initial state of interest - e.g., for the purposes of some experiment - is addressed. Three distinct methods of state preparation are described. One of these methods has the attractive feature that it enables one to prepare $S$ in a preassigned initial state with certainty; i.e., the probability of success in preparing $S$ in a given state is unity. This method relies on coupling $S$ to an open quantum-mechanical environment, $E$, in such a way that the dynamics of $S \vee E$ pulls the state of $S$ towards an "attractor", which is the desired initial state of $S$. This method is analyzed in detail.

==> Section_Graph-1.tex <==

\section{ Rewriting $\mathcal{Z}^{t,0}$ as a sum of terms labelled by graphs}
\label{graphph}
 We  rewrite the Dyson expansion for  $\mathcal{Z}^{t,0}$  using graphs labeling terms arising from partial re-summations of the Dyson series.  Our analysis contains three steps.\\
\vspace{1mm}

\noindent \textit{First step.} We discretize time on the Van Hove time scale and consider intervals $I_i:=[t_{i}, t_{i+1})$ with $t_{i+1}=t_{i} +\tau \lambda^{-2}(t_{i})$, $i=0,...,N-1$  and $t_0=0$.   We  introduce  four Feynman rules that correspond to the four possible contraction schemes  in the Dyson expansion \eqref{DD1'} and we associate a Feynman diagram to each pairing  appearing under the integrals in  \eqref{DD1'}; see Paragraph \ref{Par1}.\\
 

\noindent \textit{Second step.}   We re-sum the contributions to the Dyson series corresponding to all  diagrams  that have the property that any correlation line starting in an interval $I_i$  is ending in the \textit{same} interval $I_i$, for any $i=1,...,N$.   We observe that this re-summation just yields the contribution of the operator 
$\mathcal{Z}^{t_{i+1},t_{i}}$ to the Dyson series for $\mathcal{Z}^{t_N,0}$; see subsection \ref{suba}. \\
 

 \noindent \textit{Third step.} We use the decomposition \eqref{dec} of Lemma \ref{spectrum2}, in order to  express  $ \langle \Psi(t) \vert O  \Psi(t) \rangle$ in the form of a convergent cluster expansion. The fact that the range of the projections $P(t_i)$ is one-dimensional plays an important role. Indeed, a product of operators 
 $A_1,..., A_n \in \mathcal{B} (\mathcal{B}(\mathcal{H}_S))$, when sandwiched  between two  projections $P(s_1)=\vert 1_S \rangle \langle \Pi(s_1) \vert $ and $P(s_2)=\vert 1_S \rangle \langle \Pi(s_2) \vert$, is equal to  
 \begin{equation*}
 P(s_1)A_1... A_n P(s_2)= P(s_2)  \text{ } \langle \Pi(s_2) \vert A_1... A_n \vert 1_s \rangle. 
\end{equation*}
Using this identity, we are able to assign a  scalar weight  to each element, $\mathcal{X}$, of a set, denoted by $\mathbb{P}_{N}$, of  ``polymers''. The set  $\mathbb{P}_{N}$ is constructed from the possible pairings (correlation lines) appearing in Wick's theorem;   see subsection \ref{secon}.


\subsection{Discretization of time, and Feynman rules }
\label{Par1}
We introduce a sequence $(t_i)_{i \geq 0}$ of times with the help of a recursion formula
\begin{equation}
\label{discr}
t_{i+1}=t_i +\tau \lambda^{-2}(t_i), \qquad t_0=0.
\end{equation}
We set
\begin{align}
\label{lambda}
\lambda_i&:=\lambda(t_i),\\
\label{Ii}
I_{i}&:=\left[ t_{i}, t_{i+1}\right).
\end{align}
\input{curve}

\label{ff}
We introduce four  Feynman rules  corresponding to the four possible contractions displayed in \eqref{F2}:  
 %\input{lignetemps} 
\input{feynman}
corresponding to the ``operator-valued amplitudes''
\begin{align}
\label{fey1}
\textbf{(a)}&:=\lambda(u_i) \lambda(v_i)  f(u_i-v_i) \textbf{L}(iG(u_i)) \textbf{L}(iG(v_i)),  \\
\textbf{(b)}&:=\lambda(u_i) \lambda(v_i) f(u_i-v_i)  \textbf{L}(iG(u_i)) \textbf{R}(iG(v_i)),   \\
\textbf{(c)}&:=\lambda(u_i) \lambda(v_i) f(v_i-u_i)  \textbf{R}(iG(u_i)) \textbf{L}(iG(v_i)),   \\
\label{fey4}
\textbf{(d)}&:=\lambda(u_i) \lambda(v_i)  f(v_i-u_i) \textbf{R}(iG(u_i)) \textbf{R}(iG(v_i)).
\end{align}
The expressions (\ref{fey1})-(\ref{fey4}) can be read off directly from (\ref{F2}). To any operator 
$$ \lambda( \underline{u})  \lambda( \underline{v} )   \mathcal{T}_S \left[ \prod_{i=1}^{k}   \textbf{F}(u_{i},r_i ;v_{i},r'_i)  \right] $$
 in \eqref{DD1'} there corresponds a unique Feynman diagram constructed according to the rules (\ref{fey1})-(\ref{fey4}), above. (Time ordering has to be carried out to determine the corresponding contribution to \eqref{DD1'}).  We are led to considering  diagrams of a kind indicated in Figure 1. \input{graph2}


\newpage
\subsection{Resummation}
\label{presum}


\subsubsection{Re-summing  the Dyson expansion inside isolated double intervals }
We fix a natural number $N \in \mathbb{N}$.  To each  interval $I_i$, as defined in (\ref{Ii}), we associate an index $r$ that takes the values $0$ or $1$. We set $\textbf{I}_i:=\left(I_{i},0;I_{i},1\right)$  and call $\textbf{I}_i$ a  double interval.  It corresponds to the picture
\begin{center}
\begin{tikzpicture}[scale=0.6]

\draw[-] (1,0) -- (2.5,0);
\draw[-,] (1,-3) -- (2.5,-3);

\draw[-,thick]  (1,-0.05) -- (1,0.05);
\draw[-,thick]  (2.5,-0.05) -- (2.5,0.05);

\draw[-,thick]  (1,-3.05) -- (1,-2.95);
\draw[-,thick]  (2.5,-3.05) -- (2.5,-2.95);


 \draw (1.05,0) node[below] {$t_{i}$};
 \draw (2.55,0) node[below] {$t_{i+1}$};
 \draw (1.05,-3) node[below] {$t_{i}$};
 \draw (2.55,-3) node[below] {$t_{i+1}$};
\end{tikzpicture}
\end{center}

\noindent The curved part from $(t_N,r=0)$ to $(t_N,r=1)$ in Figure \ref{M1}, which contains a point representing the observable $O$, is  also considered to be a double interval and is denoted by  $\textbf{I}_{N}$.  There are two types of  double intervals in Figure \ref{M1}: either $\textbf{I}_i$  is  connected to  some  $\textbf{I}_j$ ($j \neq i$) by a wavy (correlation) line; or all wavy (correlation) lines starting  in  $\textbf{I}_i$ end  in  $\textbf{I}_i$. In this latter case, we say that $\textbf{I}_i$ is isolated. Let  
$\textbf{I}_{i_0}$, with $i_0 \neq N$, be an isolated interval. We re-sum the Dyson expansion inside this interval  . Let $A \subseteq \{0,...,N \}$. A function 
$\mathds{1}_{A }$  is defined on the set of all possible pairings (Wick contraction schemes) as follows:
\begin{equation}
\mathds{1}_{A}(\underline{w}):=\left\{ \begin{array}{cl}  1 & \text{ if  }  \exists i \in A \text{ such that } \textbf{I}_{i}  \text{ is isolated, }\\0 & \text{ otherwise}. \end{array} \right.
\end{equation}
In the example where $A=\{i_0\}$ we rewrite
\label{suba}
\begin{equation}
\label{DD13}
 \mathcal{Z}^{t_N,0}(O)    = \mathcal{Z}_{\{i_0\}}^{t_N,0}(O) +( \mathcal{Z}^{t_N,0}(O) -\mathcal{Z}_{\{i_0\}}^{t_N,0}(O))  \end{equation}
where
\begin{align}
\label{DD13}
 \mathcal{Z}_{\{i_0\}}^{t_N,0}(O)   & = \sum_{k=0}^{\infty}  \underset{[0,t]^{2k}}{\int} d\mu_k(\underline{w})  \lambda( \underline{w})  \text{ } \mathds{1}_{\{i_0\}}(\underline{w}) \mathcal{T}_S \left[    
  \textbf{F}( \underline{w})  \right] \left[ O_{t_N} \right].
\end{align}
To shorten our formulae, we have introduced the notation
\begin{equation}
\label{FF}
 \textbf{F}( \underline{w}) := \prod_{i=1}^{k}   {\bf{F}}(u_{i}, r_{i}; v_{i}, r'_{i}),
 \end{equation}
 and
 \begin{equation}
 \label{F}
 F( \underline{w}) := \prod_{i=1}^{k} F(u_{i}, r_{i}; v_{i}, r'_{i}),
 \end{equation}
 where ${\bf{F}}(u, r; v, r')$ has been defined in \eqref{F2} and $F(u_i,r_i;v_i,r'_i)$ in \eqref{F3}. We now explain how to split the integrations in the formula for $ \mathcal{Z}_{\{i_0\}}^{t_N,0}(O)$. Interchanging summations and integrations will be carried out without further mention, because the Dyson series converges in norm;  see $\eqref{labound}$. For every pairing $\underline{w}$ consisting of $k$ pairs, it is convenient to write
\begin{equation}
\label{1G}
\mathds{1}_{\{i_0\}}(\underline{w})=  \sum_{m=0}^{k} \mathds{1}_{\{i_0\},m} (\underline{w}),
  \end{equation}
where $ \mathds{1}_{\{i_0\},m} (\underline{w})=1$ if $\textbf{I}_{i_0}$ is isolated and contains exactly $m$ pairs, and is equal to zero otherwise. We plug (\ref{1G})  into (\ref{DD13}). This yields
\begin{equation}
\label{DD14}
\begin{split}
 \mathcal{Z}_{\{i_0\}}^{t_N,0}(O)=\sum_{k=0}^{\infty}  \sum_{m=0}^{k}  \underset{[0,t_N]^{2k}}{\int} d\mu_k (\underline{w})  \lambda( \underline{w})    \text{ } \mathds{1}_{\{i_0\} ,m}(\underline{w}) \mathcal{T}_S \Big[ \prod_{i=1}^{k}   \text{ }  {\bf{F}}(\underline{w})  \Big] \left[ O_{t_N} \right].
\end{split}
\end{equation}
Given some pairing $\underline{w}$, with $ \mathds{1}_{\{i_0\} ,m}(\underline{w}) =1,$ for some $m \in \mathbb{N}$, there are two unique pairings $\underline{\tilde{w}}$ and $\underline{\hat{w}}$,  with  $\underline{w}=\underline{\tilde{w}} \cup \underline{\hat{w}}$,  such  that \textit{all} times in $\underline{\hat{w}}$  lie in $\textbf{I}_{i_0}$, whereas  \textit{no} time in   $\underline{\tilde{w}}$ lies in $\textbf{I}_{i_0}$. After a change of variables we can factorize the integral in \eqref{DD14} into two distinct integrals. Exchanging summation over $k$ with summation over $m$, we  get that 
\begin{equation*}
%\label{DD16}
\begin{split}
\mathcal{Z}_{\{i_0\}}^{t_N,0}(O)=\sum_{k=0}^{\infty}  & \underset{[0,t_N]^{2k}}{\int} d\mu_{k}  (\underline{\tilde{w}})  \lambda( \underline{\tilde{w}})  \text{ }  \chi_{\{1,...N\} \setminus \{i_0\}}( \underline{\tilde{w}})\\
 & \mathcal{T}_S \Big(    \textbf{F}( \underline{\tilde{w}})  \sum_{m=0}^{\infty}  \underset{ I_{i_0}}{\int} d\mu_m (\underline{\hat{w}})  \lambda( \underline{\hat{w}})    \mathcal{T}_S \left[   \textbf{F}( \underline{\hat{w}})  \right] \Big) \left[ O_{t_N} \right].
 \end{split}
\end{equation*}
We recognize the expansion of the effective propagator $e^{i t_{i_{0}} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+1},t_{i_0}}e^{-i t_{i_0+1} \mathcal{L}_S}$  inside the parenthesis on the right side of this equation; see \eqref{DD1'}.  Note that $ \chi_{\{1,...N\} \setminus \{i_0\}}$  only selects pairings  with no pairs inside $\textbf{I}_{i_0}$ or linked to $\textbf{I}_{i_0}$. Repeating this procedure for each interval,  we obtain the following lemma.

\begin{lemma} 
\label{coiso}
\begin{equation}
\label{DDtt}
\begin{split}
 \mathcal{Z}^{t_N,0}(O)  = \sum_{A \subseteq \{0,...,N \} } & \sum_{k=0}^{\infty}      \underset{[0,t_N]^{2k}}{\int} d\mu_{k} (\underline{w})  \lambda( \underline{w})    \text{ }   \big(1- \mathds{1}_{\{0,...,N \} \setminus A}   (\underline{w}) \big)  \chi_{\{1,...N\} \setminus A}(\underline{w}) \\
 &\mathcal{T}_S \Big(      \textbf{F}( \underline{w} ) \text{ }  \prod_{j \in A} \big( e^{i t_{j} \mathcal{L}_S}\mathcal{Z}^{t_{j+1},t_{j}}e^{-i t_{j+1} \mathcal{L}_S} \big) \Big) \left[ O_{t_N} \right] ,
 \end{split}
\end{equation}
for all $O \in \mathcal{B}(\mathcal{H}_S)$.
\end{lemma}
\vspace{2mm}


\subsection{The cluster expansion}
\label{secon}
We plan to use the Dyson series for $\mathcal{Z}^{t,s}$ and Lemma \ref{spectrum2}, namely the identity
\begin{equation}
 \label{dec2}
 \mathcal{Z}^{t_{i+1}, t_i} = P(t_i)+R(t_i),
 \end{equation}
to  rewrite $\langle \Psi(t_N)  \vert (O  \otimes 1)   \Psi(t_N) \rangle$  in the form of a cluster- or polymer expansion. Observing that
\begin{equation*}
e^{i t_{i_{0}} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+1},t_{i_0}}e^{-i t_{i_0+1} \mathcal{L}_S} e^{i t_{i_{0}+1} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+2},t_{i_0+1}} e^{-i t_{i_0+2} \mathcal{L}_S}
=e^{i t_{i_{0}} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+1},t_{i_0}} \mathcal{Z}^{t_{i_0+2},t_{i_0+1}} e^{-i t_{i_0+2}  \mathcal{L}_S}
\end{equation*}
and that
\begin{equation*}
e^{i t_{N-1} \mathcal{L}_S} \mathcal{Z}^{t_{N},t_{N-1}} e^{-i t_{N} \mathcal{L}_S} O_{t_N}=e^{i t_{N-1} \mathcal{L}_S} \mathcal{Z}^{t_{N},t_{N-1}} O.
\end{equation*}
we see that the operators $e^{it_j \mathcal{L}_S}$  cancel each other in the product inside the parentheses in \eqref{DDtt} unless they are located at the endpoints of  a union of adjacent isolated  intervals. We   extend   the definition of the time-ordering operator $\mathcal{T}_S$   in such a way that  $\mathcal{T}_S$ places 
$e^{i t_{i_{l}} \mathcal{L}_S}$ on the left of $e^{-i t_{i_{l}} \mathcal{L}_S}$  and $e^{-i t_{i_{l}+1} \mathcal{L}_S}$ on the right of  $\mathcal{Z}^{t_{i_l+1},t_{i_l}}$. We may then write
\begin{equation}
\label{DDt}
\begin{split}
 \mathcal{Z}^{t_N,0}(O)=\sum_{A  \subseteq \{0,...,N \} }\sum_{k=0}^{\infty} &    \underset{[0,t_N]^{2k} }{\int} d\mu_{k} (\underline{w})  \lambda( \underline{w})    \text{ }   \big(1- \mathds{1}_{\{0,...,N \} \setminus A}   (\underline{w}) \big) \chi_{\{1,...N\} \setminus A}(\underline{w} )   \\
 &\mathcal{T}_S \Big(    \big( \prod_{l \in A}  e^{-i t_{i_{l}+1} \mathcal{L}_S}  \big)    \textbf{F}( \underline{w} )   \big( \prod_{l \in A}  e^{i t_{i_{l}} \mathcal{L}_S}  \big)  \big( \prod_{j \in A} \mathcal{Z}^{t_{j+1},t_{j}} \big)  \Big) [ O_{t_N} ].
 \end{split}
\end{equation} 

\noindent Next, we  insert (\ref{dec2}) into (\ref{DDt})  and expand the resulting expression as a sum of products of $P's$ and $R's$. This yields
\begin{equation}
\label{DDt2}
\begin{split}
 \mathcal{Z}^{t_N,0}(O)&=\sum_{A \subseteq \{0,...,N \}} \sum_{C \subseteq A } \sum_{k=0}^{\infty}     \underset{[0,t_N]^{2k} }{\int} d\mu_{k} (\underline{w})  \lambda( \underline{w})    \text{ }  \big(1- \mathds{1}_{\{0,...,N \} \setminus A}   (\underline{w}) \big) \chi_{\{1,...N\} \setminus A}(\underline{w} )   \\
 &\mathcal{T}_S \Big(    \big( \prod_{l \in A}  e^{-i t_{i_{l}+1} \mathcal{L}_S}  \big)    \textbf{F}( \underline{w} )   \big( \prod_{l \in A}  e^{i t_{i_{l}} \mathcal{L}_S}  \big)  \big( \prod_{j \in C} R(t_j) \big)  \big( \prod_{m \in A \setminus C} P(t_m) \big)  \Big) [ O_{t_N} ].
 \end{split}
\end{equation} 
\vspace{2mm}

\noindent

\subsubsection{Construction of the set $\mathbb{P}_{N}$}\label{PN}
We now elucidate the structure of the polymer set $\mathbb{P}_N$  that we use to re-organize the sums and integrals in \eqref{DDt2}.\\
\begin{itemize}[leftmargin=*]
  \item  We introduce ``decorated" vertices  by associating capital letters $R$ (for red), $P$ (for purple), or $B$ (for blue) to every integer $i \in \{0,...,N \}$. An integer $i$ labeled with an $R$, $(i,R)$, corresponds to the perturbation $R(t_i)$.  An integer $i$ labelled with a $P$, $(i,P)$, corresponds to the projection $P(t_i)$.  An integer $i$ labelled with a $B$, $(i,B)$, corresponds to an interval $\textbf{I}_i$ that is not isolated. In formula \eqref{DDt2} above, integers in the sets $C$ are labelled with an $R$, integers in the set $A \setminus C$ are labeled with a $P$, and integers in the sets $\{0,...,N \} \setminus A$ are labelled with a $B$. The integer $N$ (corresponding to the observable $O$) is labelled with an $R$ and is considered to be an $R$-vertex. \\ 

 \item  We introduce \textit{decorated graphs} on the the set $\{0,...,N \}$. A decorated graph $\mathcal{G}$ is a pair $(\mathcal{V}(\mathcal{G}),\mathcal{E}(\mathcal{G}))$. The vertex set  $\mathcal{V}(\mathcal{G})$  consists of $B$ and/or $R$-vertices. The edge set  $\mathcal{E}(\mathcal{G})$ consists of  edges $((i,B);(j,B))$ joining two distinct $B$-vertices.  The distance between two decorated graphs is defined by 
 \begin{equation}
\mbox{dist} \left(\mathcal{G}_1, \mathcal{G}_2\right):=\underset{i \in \mathcal{G}_1, \text{ } j \in \mathcal{G}_2}{\min}   \text{ }\vert i-j  \vert. 
\end{equation}

\item A  \textit{connected} graph is an $R$-vertex or a  decorated graph $\mathcal{G}=(\mathcal{V}(\mathcal{G}),\mathcal{E}(\mathcal{G}))$ such that  $\mathcal{V}(\mathcal{G})$ only contains $B$-vertices and such that the graph $\mathcal{G}$ is connected (in the usual sense of graph theory).\\

 \item A polymer $\mathcal{X} \in \mathbb{P}_N$ is  a union of \textit{disjoint connected} graphs  $\mathcal{G}_1,....,\mathcal{G}_n$ (for some $n \in \mathbb{N}$)  such that $\mbox{dist}\left( \cup_{j \in J}\mathcal{G}_j, \mathcal{X} \setminus (\cup_{j \in J}\mathcal{G}_j) \right) =1$, for all  $J \subseteq \{1,...,n \}$. The vertices of $\mathcal{X}$ are denoted by $\mathcal{V}(\mathcal{X})$, and the edges  by $\mathcal{E}(\mathcal{X})$.\\
 \end{itemize}



\subsubsection{The cluster expansion}
\noindent We use the  polymer set $\mathbb{P}_N$ to  rewrite the Dyson series in \eqref{DDt2} in a more convenient form. Starting from \eqref{DDt2}, with contributions corresponding to $P$- and $R$-vertices 
re-summed, we remark that the intervals $\textbf{I}_i$ corresponding to B-vertices  (where $i \in \{0,...,N \} \setminus A$) may be connected by pairings, $\underline{w}$, with  $ \mathds{1}_{\{0,...,N \} \setminus A}   (\underline{w})=0$, in many different ways.   We associate  a  decorated  graph $\mathcal{G}$  to every subset $A \subseteq \{0,...,N \}$ and to every pairing $\underline{w}$  with $ \mathds{1}_{\{0,...,N \} \setminus A}   (\underline{w})=0$ by labeling elements of $A$ by an  index $R$ or  $P$  and by drawing an edge between $(i,B)$ and  $(j,B)$  if  there is a correlation line starting in $\textbf{I}_i$  and ending in  $\textbf{I}_j$. The  decorated graph $\mathcal{G}$ can be  rewritten as a disjoint union of connected components. We fuse  the adjacent connected components of $\mathcal{G}$ and obtain a collection of non-adjacent  polymers $\mathcal{X}_1,...,\mathcal{X}_n \in  \mathbb{P}_N$, for some $n \leq N$. 
\input{graphfey}


 \noindent Summing terms in the Dyson series labelled by subsets  $A \subseteq \{0,...,N \}$,  after  integrating over all  pairings $\underline{w}$  such that  
 $\mathds{1}_{\{0,...,N \} \setminus A}   (\underline{w})=0$  in \eqref{DDt2}, amounts to the same as summing terms labelled by arbitrary collections of  non-adjacent polymers, after integrating over all pairings compatible with these polymers (pairings whose correlation lines follow the edges of the polymers). At their boundaries, polymers are surrounded by $P$-vertices (corresponding to one-dimensional projections), and the contributions corresponding to non-adjacent polymers factorize. This observation implies that the expectation value $\langle \Psi(t_N) \vert  O    \Psi(t_N) \rangle$ can be represented in the form of a cluster expansion for a one-dimensional gas of polymers, with polymers corresponding to the elements of the set $\mathbb{P}_N$.
\newpage

\begin{proposition}
\label{clustt}
\leavevmode
\begin{enumerate} 
\item There is a  complex-valued function $p: \mathbb{P}_N \rightarrow \mathbb{C}$  such that 
\begin{align}
\label{eqclu1}
\langle \Psi (t_N) \vert (O  \otimes 1)   \Psi(t_N) \rangle&=  \sum_{n=1}^{N} \frac{1}{n!} \underset{\text{dist}(\mathcal{X}_i,\mathcal{X}_j) \geq 2, \text{ } \exists i_0, \text{ } (N,R) \in \mathcal{V}( \mathcal{X}_{i_0})}{\underset{\mathcal{X}_1,...,\mathcal{X}_n \in \mathbb{P}_{N}}{\sum}}   p(\mathcal{X}_1) \text{ }... \text{ } p(\mathcal{X}_n). 
\end{align}
The weight $p(\mathcal{X})$ depends  on the observable $O$ only if $(N,R)$ is a vertex of the polymer $\mathcal{X}$.
\vspace{2mm}

\item If $\lambda(0)$  is sufficiently small,  there is  a non-negative function  $a: \mathbb{P}_N \rightarrow \mathbb{R}_+$ such that
\begin{equation} \label{kokori}
\sum_{\mathcal{X}', \text{dist}(\mathcal{X},\mathcal{X}')=1} \vert  p(\mathcal{X}') \vert e^{a(\mathcal{X}')} \leq a(\mathcal{X}), \qquad \forall \chi \in \mathbb{P}_N. 
\end{equation}
The  critical value of  $\lambda(0)$ such that  \eqref{kokori} is satisfied can be chosen  uniformly in $N$.
\end{enumerate}

\end{proposition}
\vspace{4mm}


\begin{remark}  The factors $1/n!$ on the right sides of  \eqref{eqclu1} account for over-counting that originates in summing over all permutations of the polymers $\mathcal{X}_1,...,\mathcal{X}_n$ in $\mathbb{P}_{N}$ . Clearly, the maximal number, $n$, of polymers  appearing in the sums on the right sides of Eqs. \eqref{eqclu1}
  is finite, with $n<N$.
\end{remark}

\begin{remark} \label{1.1}
Property (1) of Proposition \ref{clustt} is proven in Appendix \ref{AppC}. The proof of the Kotecky-Preiss criterion \eqref{kokori} needs some amount of work and is  given in Section \ref{sectionko}. The cluster expansion \eqref{eqclu1} can also be applied when $O$ happens to be the identity, $1_S$: \begin{align}
\label{eqclu11}
\langle \Psi (t_N) \vert (1_S  \otimes 1)   \Psi(t_N) \rangle&=  \sum_{n=1}^{N} \frac{1}{n!} \underset{\text{dist}(\mathcal{X}_i,\mathcal{X}_j) \geq 2, \text{ } \exists i_0, \text{ } (N,R) \in \mathcal{V}( \mathcal{X}_{i_0})}{\underset{\mathcal{X}_1,...,\mathcal{X}_n \in \mathbb{P}_{N}}{\sum}}   p(\mathcal{X}_1) \text{ }... \text{ } p(\mathcal{X}_n), 
\end{align}
and the weights $p(\mathcal{X})$ depends on $1_S$ only if $(N,R)$ is a vertex of the polymer $\mathcal{X}$.  The right side of \eqref{eqclu2} is then equal to 1, because the initial state $\vert  \Psi \rangle$ is assumed to be normalized. An interesting property, inherent to our cluster expansion,  relies in the fact that we can  rewrite \eqref{eqclu1} by restricting the sum in \eqref{eqclu1} to  collections of  polymers that do not contain the vertex $(N,R)$:
\begin{align}
\label{eqclu2}
\langle \Psi (t_N) \vert (1_S  \otimes 1)   \Psi(t_N) \rangle&=   1+ \sum_{n=1}^{N} \frac{1}{n!} \underset{\text{dist}(\mathcal{X}_i,\mathcal{X}_j) \geq 2, \text{ }(N,R) \notin \cup_i \mathcal{V}( \mathcal{X}_{i})}{\underset{\mathcal{X}_1,...,\mathcal{X}_n \in \mathbb{P}_{N}}{\sum}}   p(\mathcal{X}_1)...p(\mathcal{X}_n).
\end{align}
We rapidly sketch the proof of \eqref{eqclu2}. We first split the sum in \eqref{eqclu11} into two terms, distinguishing whether or not the polymer $\mathcal{X}_{i_0}$  is equal to $\{(N,R)\}$. If $\mathcal{X}_{i_0}=\{(N,R)\}$, then 
\begin{equation}
p(\mathcal{X}_1)...  p(\mathcal{X}_{i_0-1}) p(\mathcal{X}_{i_0})  p(\mathcal{X}_{i_0-1}) ... p(\mathcal{X}_n)=p(\mathcal{X}_1) ...  p(\mathcal{X}_{i_0-1})  p(\mathcal{X}_{i_0-1})  ...p(\mathcal{X}_n)
\end{equation} 
because $p(\{(N,R)\})=\langle \varphi \vert  \varphi \rangle \text{Tr} (\Pi(t_N))=1$ if  $O=1_S$.  Moreover, the other polymers are located at a distance greater or equal  to 2 from the polymer $\{(N,R)\}$, and they cannot contain the vertices $(N,R)$ and $(N-1,\cdot)$. This remark leads to an obvious simplification on the right side of \eqref{eqclu11} for collections of polymers such that $\mathcal{X}_{i_0}=\{(N,R)\}$. Their contribution is just equal to 
\begin{equation}
\label{eqclu122}
 1+ \sum_{n=1}^{N} \frac{1}{n!}  \quad \underset{(N,R), (N-1,\cdot) \notin \cup_i \mathcal{V}( \mathcal{X}_{i})}{\underset{\mathcal{X}_1,...,\mathcal{X}_n \in \mathbb{P}_{N}, \text{ dist}(\mathcal{X}_i,\mathcal{X}_j) \geq 2,}{\sum}}   p(\mathcal{X}_1)...p(\mathcal{X}_n).
\end{equation}
If  $\mathcal{X}_{i_0} \neq \{(N,R)\}$ on the right side of \eqref{eqclu11}, then we remark (see \eqref{p(G)} and \eqref{hU} below)  that the contribution of the vertex $(N,R)$ to $p(\mathcal{X}_{i_0})$ is trivial since it corresponds to a left multiplication by the identity operator $1_S$.  Moreover, $\mathcal{X}_{i_0} $ must contain the vertex $(N-1,\cdot)$ since $\mathcal{X}_{i_0}$  is a polymer (a fusion of adjacent connected graphs). We can therefore erase the vertex $(N,R)$ from the polymer $\mathcal{X}_{i_0}$. The other polymers are located at a distance greater or equal to 2 from $\mathcal{X}_{i_0}$, and the contribution of the  collections of polymers such that $\mathcal{X}_{i_0} \neq \{(N,R)\}$  in the sum in  \eqref{eqclu11} is equal to 
\begin{equation} \label{eqclu123}
\sum_{n=1}^{N} \frac{1}{n!} \quad \underset{ \tiny \begin{array}{cc} &(N,R) \notin \cup_i \mathcal{V}( \mathcal{X}_{i})\\
& \text{ }\exists i_0, \text{ } (N-1,\cdot) \in \mathcal{V}( \mathcal{X}_{i_0})\end{array} }{\underset{\mathcal{X}_1,...,\mathcal{X}_n \in \mathbb{P}_{N},  \text{ dist}(\mathcal{X}_i,\mathcal{X}_j) \geq 2,}{\sum}}   p(\mathcal{X}_1)...p(\mathcal{X}_n)
\end{equation}
Adding \eqref{eqclu122} to  \eqref{eqclu123} leads to \eqref{eqclu2}.
\end{remark}

\begin{remark}  The cluster expansion converges in the limit where $N \rightarrow \infty$, because the coupling function $\lambda(t)$ is small, for all  times $t$, and because the two-point correlation function $f(t)$ is ``twice integrable''. We investigate this limit in Section \ref{conv}.
\end{remark}

We conclude this section by introducing some useful notions and  notations that enable us to write the exact expressions for  the weights $p(\cdot)$. Let $\mathcal{X}$ be a polymer. We say that a  set $U=\{(i,.),(i+1,.),...,(i+k,.)\} \subseteq \mathcal{V}(\mathcal{X})$  is  a \textit{maximal block} of neighboring  vertices  if there is no  set $V \subseteq \mathcal{V}(\mathcal{X})$ of  neighboring  vertices such that $ U \subsetneq V$. We denote by  
$\mathcal{U}(\mathcal{X})$ the set of maximal blocks of neighboring vertices  of  $\mathcal{X}$.  Maximal blocks of neighboring vertices are  surrounded at their boundaries (extreme points) by vertices corresponding to double intervals where a one-dimensional projection $P$ is chosen. The notion of ``maximal blocks of neighboring vertices'' is therefore helpful in the formulation of the cluster expansion \eqref{eqclu1} and the weights $p(\mathcal{X)}$. We prove in Appendix \ref{AppC} that 
\begin{equation}
\label{p(G)}
p(\mathcal{X}):=\sum_{k=0}^{\infty }  \underset{[0,t_N]^{2k}} {\int} d\mu_k  (\underline{w})  \lambda( \underline{w})    \text{ }   \chi_{\mathcal{X} } (\underline{w})  \text{ F}(\underline{w})   \prod_{U \in \mathcal{U}(\mathcal{X})} h_U(\underline{w}),
\end{equation}
with
\begin{equation}
\label{hU}
 h_U(\underline{w}):=\langle \Pi (t_{m(U)}) \vert \mathcal{T}_S \Big( \underset{(i,B) \in U  }{\prod} \Big[ e^{-it_{i} \mathcal{L}_S} \big( \prod_{(t,r) \in  \underline{w} \cap \textbf{I}_i } (i G)(t,r) \big) e^{it_{i+1} \mathcal{L}_S} \Big]   \underset{(j,R) \in U  }{\prod} R(t_j) \Big) 1_S \rangle,
\end{equation}
 and where we have set  
 \begin{equation}
 \label{mmm}
 \Pi(t_{-1}):= \vert \varphi  \rangle \langle \varphi \vert, \qquad  R(t_{N}):=\textbf{L}(O), \qquad \text{and} \qquad m(U):= \min \{  i \mid (i, \cdot) \in U \}-1.
 \end{equation}
The function $ \chi_{\mathcal{X}} (\underline{w})$ is equal to $1$ only  for pairings $\underline{w}$ that are compatible with the edges of  $\mathcal{X}$ (in the sense that the correlation lines of $\underline{w}$ follow the edges of $\mathcal{X}$). It takes the value zero otherwise. 
\vspace{2mm}











==> Section_Graph-2.tex <==

\section{ Rewriting $\mathcal{Z}^{t,0}$ as a sum over connected graphs}
\label{graphph}
 We  rewrite the Dyson expansion for  $\mathcal{Z}^{t,0}$  using graphs.  Our analysis contains three steps.\\
\vspace{1mm}

\noindent \textit{First step.} We discretize time on the Van Hove time scale and consider intervals $I_i:=[t_{i}, t_{i+1})$ with $t_{i+1}=t_{i} +\tau \lambda^{-2}(t_{i})$, $i=0,...,N-1$  and $t_0=0$.   We  introduce  four Feynman rules that correspond to the four possible contraction schemes  in the Dyson expansion \eqref{DD1'} and we associate a Feynman diagram to each pairing  appearing under the integrals in  \eqref{DD1'}; see Paragraph \ref{Par1}.\\
 

\noindent \textit{Second step.}   We re-sum the contributions to the Dyson series corresponding to all  diagrams  that have the property that any correlation line starting in an interval $I_i$  is ending in the \textit{same} interval $I_i$, for any $i=1,...,N$.   We observe that this re-summation just yields the contribution of the operator 
$\mathcal{Z}^{t_{i+1},t_{i}}$ to the Dyson series for $\mathcal{Z}^{t_N,0}$; see subsection \ref{suba}. \\
 

 \noindent \textit{Third step.} We use the decomposition \eqref{dec} of Lemma \ref{spectrum2}, in order to  express  $ \langle \Psi(t) \vert O  \Psi(t) \rangle$ in the form of a convergent cluster expansion. The fact that the range of the projections $P(t_i)$ is one-dimensional plays an important role. Indeed, a product of operators 
 $A_1,..., A_n \in \mathcal{B} (\mathcal{B}(\mathcal{H}_S))$, when sandwiched  between two  projections $P(s_1)=\vert 1_S \rangle \langle \Pi(s_1) \vert $ and $P(s_2)=\vert 1_S \rangle \langle \Pi(s_2) \vert$, is equal to  
 \begin{equation*}
 P(s_1)A_1... A_n P(s_2)= P(s_2)  \text{ } \langle \Pi(s_2) \vert A_1... A_n \vert 1_s \rangle. 
\end{equation*}
Using this identity, we are able to assign a  scalar weight  to each element, $\mathcal{X}$, of a set, denoted by $\mathbb{P}_{N}$, of  ``polymers''. The set  $\mathbb{P}_{N}$ is constructed from the possible pairings (correlation lines) appearing in Wick's theorem;   see subsection \ref{secon}.


\subsection{Discretization of time, and Feynman rules }
\label{Par1}
We introduce a sequence $(t_i)_{i \geq 0}$ of times with the help of a recursion formula
\begin{equation}
\label{discr}
t_{i+1}=t_i +\tau \lambda^{-2}(t_i), \qquad t_0=0.
\end{equation}
We set
\begin{align}
\label{lambda}
\lambda_i&:=\lambda(t_i),\\
\label{Ii}
I_{i}&:=\left[ t_{i}, t_{i+1}\right).
\end{align}
\input{curve}

\label{ff}
We introduce four  Feynman rules  corresponding to the four possible contractions displayed in \eqref{F2}:  
 %\input{lignetemps} 
\input{feynman}
corresponding to the ``operator-valued amplitudes''
\begin{align}
\label{fey1}
\textbf{(a)}&:=\lambda(u_i) \lambda(v_i)  f(u_i-v_i) \textbf{L}(iG(u_i)) \textbf{L}(iG(v_i)),  \\
\textbf{(b)}&:=\lambda(u_i) \lambda(v_i) f(u_i-v_i)  \textbf{L}(iG(u_i)) \textbf{R}(iG(v_i)),   \\
\textbf{(c)}&:=\lambda(u_i) \lambda(v_i) f(v_i-u_i)  \textbf{R}(iG(u_i)) \textbf{L}(iG(v_i)),   \\
\label{fey4}
\textbf{(d)}&:=\lambda(u_i) \lambda(v_i)  f(v_i-u_i) \textbf{R}(iG(u_i)) \textbf{R}(iG(v_i)).
\end{align}
The expressions (\ref{fey1})-(\ref{fey4}) can be read off directly from (\ref{F2}). To any operator 
$$ \lambda( \underline{u})  \lambda( \underline{v} )   \mathcal{T}_S \left[ \prod_{i=1}^{k}   \textbf{F}(u_{i},r_i ;v_{i},r'_i)  \right] $$
 in \eqref{DD1'} there corresponds a unique Feynman diagram constructed according to the rules (\ref{fey1})-(\ref{fey4}), above. (Time ordering has to be carried out to determine the corresponding contribution to \eqref{DD1'}).  We are led to considering  diagrams of a kind indicated in Figure 1. \input{graph2}


\newpage
\subsection{Resummation}
\label{presum}


\subsubsection{Re-summing  the Dyson expansion inside isolated double intervals }
We fix a natural number $N \in \mathbb{N}$.  To each  interval $I_i$, as defined in (\ref{Ii}), we associate an index $r$ that takes the values $0$ or $1$. We set $\textbf{I}_i:=\left(I_{i},0;I_{i},1\right)$  and call $\textbf{I}_i$ a  double interval.  It corresponds to the picture
\begin{center}
\begin{tikzpicture}[scale=0.6]

\draw[-] (1,0) -- (2.5,0);
\draw[-,] (1,-3) -- (2.5,-3);

\draw[-,thick]  (1,-0.05) -- (1,0.05);
\draw[-,thick]  (2.5,-0.05) -- (2.5,0.05);

\draw[-,thick]  (1,-3.05) -- (1,-2.95);
\draw[-,thick]  (2.5,-3.05) -- (2.5,-2.95);


 \draw (1.05,0) node[below] {$t_{i}$};
 \draw (2.55,0) node[below] {$t_{i+1}$};
 \draw (1.05,-3) node[below] {$t_{i}$};
 \draw (2.55,-3) node[below] {$t_{i+1}$};
\end{tikzpicture}
\end{center}

\noindent The curved part from $(t_N,r=0)$ to $(t_N,r=1)$ in Figure \ref{M1}, which contains a point representing the observable $O$, is  also considered to be a double interval and is denoted by  $\textbf{I}_{N}$.  There are two types of  double intervals in Figure \ref{M1}: either $\textbf{I}_i$  is  connected to  some  $\textbf{I}_j$ ($j \neq i$) by a wavy (correlation) line; or all wavy (correlation) lines starting  in  $\textbf{I}_i$ end  in  $\textbf{I}_i$. In this latter case, we say that $\textbf{I}_i$ is isolated. Let  
$\textbf{I}_{i_0}$, with $i_0 \neq N$, be an isolated interval. We re-sum the Dyson expansion inside this interval  . Let $A \subseteq \{0,...,N \}$. A function 
$\mathds{1}_{A }$  is defined on the set of all possible pairings (Wick contraction schemes) as follows:
\begin{equation}
\mathds{1}_{A}(\underline{w}):=\left\{ \begin{array}{cl}  1 & \text{ if  }  \exists i \in A \text{ such that } \textbf{I}_{i}  \text{ is isolated, }\\0 & \text{ otherwise}. \end{array} \right.
\end{equation}
In the example where $A=\{i_0\}$ we rewrite \\
{\red{here comes a really bad notation!!!}}
\label{suba}
\begin{equation}
\label{DD13}
 \mathcal{Z}^{t_N,0}(O)    = \mathcal{Z}_{\{i_0\}}^{t_N,0}(O) + \mathcal{Z}_{\overline{\{i_0\}}}^{t_N,0}(O)
\end{equation}
where
\begin{align}
\label{DD13}
 \mathcal{Z}_{\{i_0\}}^{t_N,0}(O)   & = \sum_{k=0}^{\infty}  \underset{[0,t]^{2k}}{\int} d\mu_k(\underline{w})  \lambda( \underline{w})  \text{ } \mathds{1}_{\{i_0\}}(\underline{w}) \mathcal{T}_S \left[    
  \textbf{F}( \underline{w})  \right] \left[ O_{t_N} \right],\\
  \label{DD133}
 \mathcal{Z}_{\overline{\{i_0\}}}^{t_N,0}(O)&=\sum_{k=0}^{\infty}  \underset{[0,t]^{2k}}{\int} d\mu_k(\underline{w})  \lambda( \underline{w})  \text{ } (1- \mathds{1}_{\{i_0\}}(\underline{w})) \mathcal{T}_S \left[    
  \textbf{F}( \underline{w})  \right] \left[ O_{t_N} \right].
\end{align}
To shorten our formulae, we have introduced the notation
\begin{equation}
\label{FF}
 \textbf{F}( \underline{w}) := \prod_{i=1}^{k}   {\bf{F}}(u_{i}, r_{i}; v_{i}, r'_{i}),
 \end{equation}
 and
 \begin{equation}
 \label{F}
 F( \underline{w}) := \prod_{i=1}^{k} F(u_{i}, r_{i}; v_{i}, r'_{i}),
 \end{equation}
 where $F(u_{i}, r_{i}; v_{i}, r'_{i})$ has been defined in \eqref{F3}. We now explain how to split the integration in $ \mathcal{Z}_{\{i_0\}}^{t_N,0}(O)$. Interchanging summations and integrations  is  carried out without further mention, because the Dyson series converges in norm;  see $\eqref{labound}$. For every pairing $\underline{w}$ consisting of $k$ pairs, it is convenient to write
\begin{equation}
\label{1G}
\mathds{1}_{\{i_0\}}(\underline{w})=  \sum_{m=0}^{k} \mathds{1}_{\{i_0\},m} (\underline{w}),
  \end{equation}
where $ \mathds{1}_{\{i_0\},m} (\underline{w})=1$ if $\textbf{I}_{i_0}$ is isolated and contains exactly $m$ pairs, and is equal to zero otherwise. We plug (\ref{1G})  into (\ref{DD13}). This yields
\begin{equation}
\label{DD14}
\begin{split}
 \mathcal{Z}_{\{i_0\}}^{t_N,0}(O)=\sum_{k=0}^{\infty}  \sum_{m=0}^{k}  \underset{[0,t_N]^{2k}}{\int} d\mu_k (\underline{w})  \lambda( \underline{w})    \text{ } \mathds{1}_{\{i_0\} ,m}(\underline{w}) \mathcal{T}_S \Big[ \prod_{i=1}^{k}   \text{ }  {\bf{F}}(\underline{w})  \Big] \left[ O_{t_N} \right].
\end{split}
\end{equation}
Given some pairing $\underline{w}$, with $ \mathds{1}_{\{i_0\} ,m}(\underline{w}) =1,$ for some $m \in \mathbb{N}$, there are two unique pairings $\underline{\tilde{w}}$ and $\underline{\hat{w}}$,  with  $\underline{w}=\underline{\tilde{w}} \cup \underline{\hat{w}}$,  such  that \textit{all} times in $\underline{\hat{w}}$  lie in $\textbf{I}_{i_0}$, whereas  \textit{no} time in   $\underline{\tilde{w}}$ lies in $\textbf{I}_{i_0}$. After a change of variables we can factorize the integral in \eqref{DD14} into two distinct integrals. Exchanging summation over $k$ with summation over $m$, we  get that 
\begin{equation*}
%\label{DD16}
\begin{split}
\mathcal{Z}_{\{i_0\}}^{t_N,0}(O)=\sum_{k=0}^{\infty}  & \underset{[0,t_N]^{2k}}{\int} d\mu_{k}  (\underline{\tilde{w}})  \lambda( \underline{\tilde{w}})  \text{ }  \chi_{\{1,...N\} \setminus \{i_0\}}( \underline{\tilde{w}})\\
 & \mathcal{T}_S \Big(    \textbf{F}( \underline{\tilde{w}})  \sum_{m=0}^{\infty}  \underset{ I_{i_0}}{\int} d\mu_m (\underline{\hat{w}})  \lambda( \underline{\hat{w}})    \mathcal{T}_S \left[   \textbf{F}( \underline{\hat{w}})  \right] \Big) \left[ O_{t_N} \right].
 \end{split}
\end{equation*}
We recognize the expansion of the effective propagator $e^{i t_{i_{0}} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+1},t_{i_0}}e^{-i t_{i_0+1} \mathcal{L}_S}$  inside the parenthesis on the right side of this equation; see \eqref{DD1'}.  Note that $ \chi_{\{1,...N\} \setminus \{i_0\}}$  only selects pairings  with no pairs inside $\textbf{I}_{i_0}$ or linked to $\textbf{I}_{i_0}$. Repeating this procedure for each interval,  we obtain the following lemma.

\begin{lemma} 
\label{coiso}
\begin{equation}
\label{DDtt}
\begin{split}
 \mathcal{Z}^{t_N,0}(O)  = \sum_{A \subseteq \{0,...,N \} } & \sum_{k=0}^{\infty}      \underset{[0,t_N]^{2k}}{\int} d\mu_{k} (\underline{w})  \lambda( \underline{w})    \text{ }   \big(1- \mathds{1}_{\{0,...,N \} \setminus A}   (\underline{w}) \big)  \chi_{\{1,...N\} \setminus A}(\underline{w}) \\
 &\mathcal{T}_S \Big(      \textbf{F}( \underline{w} ) \text{ }  \prod_{j \in A} \big( e^{i t_{j} \mathcal{L}_S}\mathcal{Z}^{t_{j+1},t_{j}}e^{-i t_{j+1} \mathcal{L}_S} \big) \Big) \left[ O_{t_N} \right] ,
 \end{split}
\end{equation}
for all $O \in \mathcal{B}(\mathcal{H}_S)$.
\end{lemma}

\newpage
\subsection{The cluster expansion}
\label{secon}
We plan to use Lemma \ref{spectrum2}, namely the identity
\begin{equation}
 \label{dec2}
 \mathcal{Z}^{t_{i+1}, t_i} = P(t_i)+R(t_i),
 \end{equation}
to  rewrite $\langle \Psi(t_N)  \vert (O  \otimes 1)   \Psi(t_N) \rangle$  in the form of a cluster- or polymer expansion. Observing that
\begin{equation*}
e^{i t_{i_{0}} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+1},t_{i_0}}e^{-i t_{i_0+1} \mathcal{L}_S} e^{i t_{i_{0}+1} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+2},t_{i_0+1}} e^{-i t_{i_0+2} \mathcal{L}_S}
=e^{i t_{i_{0}} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+1},t_{i_0}} \mathcal{Z}^{t_{i_0+2},t_{i_0+1}} e^{-i t_{i_0+2}  \mathcal{L}_S}
\end{equation*}
and that
\begin{equation*}
e^{i t_{N-1} \mathcal{L}_S} \mathcal{Z}^{t_{N},t_{N-1}} e^{-i t_{N} \mathcal{L}_S} O_{t_N}=e^{i t_{N-1} \mathcal{L}_S} \mathcal{Z}^{t_{N},t_{N-1}} O.
\end{equation*}
we see that the operators $e^{it_j \mathcal{L}_S}$  cancel each other in the product inside the parentheses in \eqref{DDtt} unless they are located at the endpoints of  a union of adjacent isolated  intervals. We   extend   the definition of the time-ordering operator $\mathcal{T}_S$   in such a way that  $\mathcal{T}_S$ places 
$e^{i t_{i_{l}} \mathcal{L}_S}$ on the left of $e^{-i t_{i_{l}} \mathcal{L}_S}$  and $e^{-i t_{i_{l}+1} \mathcal{L}_S}$ on the right of  $\mathcal{Z}^{t_{i_l+1},t_{i_l}}$. We may then write
\begin{equation}
\label{DDt}
\begin{split}
 \mathcal{Z}^{t_N,0}(O)=\sum_{A  \subseteq \{0,...,N \} }\sum_{k=0}^{\infty} &    \underset{[0,t_N]^{2k} }{\int} d\mu_{k} (\underline{w})  \lambda( \underline{w})    \text{ }   \big(1- \mathds{1}_{\{0,...,N \} \setminus A}   (\underline{w}) \big) \chi_{\{1,...N\} \setminus A}(\underline{w} )   \\
 &\mathcal{T}_S \Big(    \big( \prod_{l \in A}  e^{-i t_{i_{l}+1} \mathcal{L}_S}  \big)    \textbf{F}( \underline{w} )   \big( \prod_{l \in A}  e^{i t_{i_{l}} \mathcal{L}_S}  \big)  \big( \prod_{j \in A} \mathcal{Z}^{t_{j+1},t_{j}} \big)  \Big) [ O_{t_N} ].
 \end{split}
\end{equation} 

\noindent Next, we  insert (\ref{dec2}) into (\ref{DDt})  and expand the resulting expression as a sum of products of $P's$ and $R's$. This yields
\begin{equation}
\label{DDt2}
\begin{split}
 \mathcal{Z}^{t_N,0}(O)&=\sum_{A \subseteq \{0,...,N \}} \sum_{C \subseteq A } \sum_{k=0}^{\infty}     \underset{[0,t_N]^{2k} }{\int} d\mu_{k} (\underline{w})  \lambda( \underline{w})    \text{ }  \big(1- \mathds{1}_{\{0,...,N \} \setminus A}   (\underline{w}) \big) \chi_{\{1,...N\} \setminus A}(\underline{w} )   \\
 &\mathcal{T}_S \Big(    \big( \prod_{l \in A}  e^{-i t_{i_{l}+1} \mathcal{L}_S}  \big)    \textbf{F}( \underline{w} )   \big( \prod_{l \in A}  e^{i t_{i_{l}} \mathcal{L}_S}  \big)  \big( \prod_{j \in C} R(t_j) \big)  \big( \prod_{m \in A \setminus C} P(t_m) \big)  \Big) [ O_{t_N} ].
 \end{split}
\end{equation} 
\vspace{2mm}

\noindent

\subsubsection{Construction of the set $\mathbb{P}_{N}$}\label{PN}
We now elucidate the structure of the polymer set $\mathbb{P}_N$  that we use to re-organize the sums and integrals in \eqref{DDt2}.\\
\begin{itemize}[leftmargin=*]
  \item  We introduce ``decorated" vertices  by associating capital letters $R$ (for red), $P$ (for purple), or $B$ (for blue) to every integer $i \in \{0,...,N \}$. An integer $i$ labeled with an $R$, $(i,R)$, corresponds to the perturbation $R(t_i)$.  An integer $i$ labelled with a $P$, $(i,P)$, corresponds to the projection $P(t_i)$.  An integer $i$ labelled with a $B$, $(i,B)$, corresponds to an interval $\textbf{I}_i$ that is not isolated. In formula \eqref{DDt2} above, integers in the sets $C$ are labelled with an $R$, integers in the set $A \setminus C$ are labeled with a $P$, and integers in the sets $\{0,...,N \} \setminus A$ are labelled with a $B$. The integer $N$ (corresponding to the observable $O$) is labelled with an $R$ and is considered to be an $R$-vertex. \\ 

 \item  We introduce \textit{decorated graphs} on the the set $\{0,...,N \}$. A decorated graph $\mathcal{G}$ is a pair $(\mathcal{V}(\mathcal{G}),\mathcal{E}(\mathcal{G}))$. The vertex set  $\mathcal{V}(\mathcal{G})$  consists of $B$ and/or $R$-vertices. The edge set  $\mathcal{E}(\mathcal{G})$ consists of  edges $((i,B);(j,B))$ joining two distinct $B$-vertices.  The distance between two decorated graphs is defined by 
 \begin{equation}
\mbox{dist} \left(\mathcal{G}_1, \mathcal{G}_2\right):=\underset{i \in \mathcal{G}_1, \text{ } j \in \mathcal{G}_2}{\min}   \text{ }\vert i-j  \vert. 
\end{equation}

\item A  \textit{connected} graph is an $R$-vertex or a  decorated graph $\mathcal{G}=(\mathcal{V}(\mathcal{G}),\mathcal{E}(\mathcal{G}))$ such that  $\mathcal{V}(\mathcal{G})$ only contains $B$-vertices and such that the graph $\mathcal{G}$ is connected (in the usual sense of graph theory).\\

 \item A polymer $\mathcal{X} \in \mathbb{P}_N$ is  a union of \textit{disjoint connected} graphs  $\mathcal{G}_1,....,\mathcal{G}_n$ (for some $n \in \mathbb{N}$)  such that $\mbox{dist}\left( \cup_{j \in J}\mathcal{G}_j, \mathcal{X} \setminus (\cup_{j \in J}\mathcal{G}_j) \right) =1$, for all  $J \subseteq \{1,...,n \}$. The vertices of $\mathcal{X}$ are denoted by $\mathcal{V}(\mathcal{X})$, and the edges  by $\mathcal{E}(\mathcal{X})$.\\
 \end{itemize}



\subsubsection{The cluster expansion}
\noindent We use the  polymer set $\mathbb{P}_N$ to  rewrite the Dyson series in \eqref{DDt2} in a more convenient form. Starting from \eqref{DDt2}, with contributions corresponding to P- and R-vertices 
re-summed, we remark that the intervals $\textbf{I}_i$ corresponding to B-vertices  (where $i \in \{0,...,N \} \setminus A$) may be connected by pairings, $\underline{w}$, with  $ \mathds{1}_{\{0,...,N \} \setminus A}   (\underline{w})=0$, in many different ways.   We associate  a  decorated  graph $\mathcal{G}$  to every subset $A \subseteq \{0,...,N \}$ and to every pairing $\underline{w}$  with $ \mathds{1}_{\{0,...,N \} \setminus A}   (\underline{w})=0$ by labeling elements of $A$ by an  index $R$ or  $P$  and by drawing an edge between $(i,B)$ and  $(j,B)$  if  there is a correlation line starting in $\textbf{I}_i$  and ending in  $\textbf{I}_j$. The  decorated graph $\mathcal{G}$ can be  rewritten as a disjoint union of connected components. We fuse  the adjacent connected components of $\mathcal{G}$ and obtain a collection of non-adjacent  polymers $\mathcal{X}_1,...,\mathcal{X}_n \in  \mathbb{P}_N$, for some $n \leq N$. 
\input{graphfey}


 \noindent Summing terms in the Dyson series labelled by subsets  $A \subseteq \{0,...,N \}$,  after  integrating over all  pairings $\underline{w}$  such that  
 $\mathds{1}_{\{0,...,N \} \setminus A}   (\underline{w})=0$  in \eqref{DDt2}, amounts to the same as summing terms labelled by arbitrary collections of  non-adjacent polymers, after integrating over all pairings compatible with these polymers (pairings whose correlation lines follow the edges of the polymers). At their boundaries, polymers are surrounded by $P$-vertices (corresponding to one-dimensional projections), and the contributions corresponding to non-adjacent polymers factorize. This observation implies that the expectation value $\langle \Psi(t_N) \vert  O    \Psi(t_N) \rangle$ can be represented in the form of a cluster expansion for a one-dimensional gas of polymers, with polymers corresponding to the elements of the set $\mathbb{P}_N$.


\begin{proposition}
\label{clustt}
There is a  complex-valued function $\zeta$ on the family of tuples of non-adjacent polymers such that 
\begin{align}
\label{eqclu1}
\langle \Psi (t_N) \vert (O  \otimes 1)   \Psi(t_N) \rangle&=  \sum_{n=1}^{N} \frac{1}{n!} \underset{\text{dist}(\mathcal{X}_i,\mathcal{X}_j) \geq 2, \text{ } \exists i_0, \text{ } (N,R) \in \mathcal{V}( \mathcal{X}_{i_0})}{\underset{\mathcal{X}_1,...,\mathcal{X}_n \in \mathbb{P}_{N}}{\sum}}   \zeta(\mathcal{X}_1,...,\mathcal{X}_n). 
\end{align}
The function $\zeta$ is symmetric in its arguments, $\mathcal{X}_i$, $i=1,2,...$, and has the following properties:\\

\begin{enumerate}
\item For arbitrary $n\in \mathbb{N}$ and arbitrary polymers $\mathcal{X}_i$, the function 
$\zeta(\mathcal{X}_1,...,\mathcal{X}_n)$ is a product of ``weights'', $p(\mathcal{X}_i), i=1,...,n$, i.e.,

\begin{equation}
\zeta(\mathcal{X}_1,...,\mathcal{X}_n)= \prod_{i=1}^{n} p(\mathcal{X}_i). 
\end{equation}
The weight $p(\mathcal{X})$ depends  on the observable $O$ only if $(N,R)$ is a vertex of the polymer $\mathcal{X}$.\\


\item  {\red{The following formulation is very awkward}}There are  a non-negative function  $a: \mathbb{P}_N \rightarrow \mathbb{R}_+$, a constant $\tau_c>0$ and a function $\lambda_{\tau}$  such that, for any 
$\tau>\tau_c$ and for any $0<\lambda(0)<\lambda_{\tau}$, the function $p$ satisfies a Kotecky-Preiss criterion: 
\begin{equation} \label{kokori}
\sum_{\mathcal{X}', \text{dist}(\mathcal{X},\mathcal{X}')=1} \vert  p(\mathcal{X}') \vert e^{a(\mathcal{X}')} \leq a(\mathcal{X}), \qquad \forall \chi \in \mathbb{P}_N. 
\end{equation}
Furthermore, $a(\cdot)$, $\tau_c$ and $\lambda_{\tau}$ do not depend on $N$.
\end{enumerate}

\end{proposition}
\vspace{4mm}



\begin{remark}  The factors $1/n!$ on the right sides of  \eqref{eqclu1} account for over-counting that originates in summing over all permutations of the polymers $\mathcal{X}_1,...,\mathcal{X}_n$ in $\mathbb{P}_{N}$ . Clearly, the maximal number, $n$, of polymers  appearing in the sums on the right sides of Eqs. \eqref{eqclu1}
  is finite, with $n<N$.
\end{remark}

\begin{remark}
Property (1) of Proposition \ref{clustt} is proven in Appendix \ref{AppC}. The proof of the Kotecky-Preiss criterion \eqref{kokori} needs some amount of work and is  given in Section \ref{sectionko}. The cluster expansion \eqref{eqclu1} can also be applied when $O$ happens to be the identity, $1_S$: 
\begin{align}
\label{eqclu2}
\langle \Psi (t_N) \vert (1_S  \otimes 1)   \Psi(t_N) \rangle&=   1+ \sum_{n=1}^{N} \frac{1}{n!} \underset{\text{dist}(\mathcal{X}_i,\mathcal{X}_j) \geq 2, \text{ }(N,R) \notin \cup_i \mathcal{V}( \mathcal{X}_{i})}{\underset{\mathcal{X}_1,...,\mathcal{X}_n \in \mathbb{P}_{N}}{\sum}}   p(\mathcal{X}_1)...p(\mathcal{X}_n). 
\end{align}
The right side of \eqref{eqclu2} is then equal to 1, because the initial state $\vert  \Psi \rangle$ is assumed to be normalized.
\end{remark}

\begin{remark}  The cluster expansion converges in the limit where $N \rightarrow \infty$, because the coupling function $\lambda(t)$ is small, for all  times $t$, and because the two-point correlation function $f(t)$ is ``twice integrable''. We investigate this limit in Section \ref{conv}.
\end{remark}

We conclude this section by introducing some useful notions and  notations that enable us to write the exact expressions for  the weights $p(\cdot)$. Given any decorated set 
$$A=\{(i_1, r_{i_1}),..., (i_n, r_{i_n})\}, \text{with} \text{   }i_j \in \{0,...,N\} \text{   } \text{and} \text{    }r_{i_j} \in \{R,P,B\}, \forall j,$$
we define
\begin{align}
\label{mmm}
m(A)&:= \min \{  i \mid (i, \cdot) \in A \}-1,\\
\label{MMM}
M(A)&:=\max \{ i \mid (i, \cdot) \in A \}+1.
\end{align}
We introduce the notion of \textit{maximal union of adjacent vertices }. Let $\mathcal{X}$ be a polymer. We say that a  set $\{(i,.),(i+1,.)...,(i+k,.)\} \subseteq \mathcal{V}(\mathcal{X})$ of  adjacent vertices is  a \textit{maximal union} of adjacent vertices  {\red{(voil\`a un bordel!!!)}} if  there is no $j<i$ or no $l>k$ such that $\{(j,.),(j+1,.)...,(j+l,.)\}$ is also contained in $ \mathcal{V}(\mathcal{X})$; (here $i,k \in \{0,...,N \}$ with $i+k \leq N$, and ``." stands for the colors $R$ or $B$).  We denote by  
$\mathcal{U}(\mathcal{X})$ the set of maximal unions of adjacent vertices  of  $\mathcal{X}$.  Maximal unions of adjacent vertices are  surrounded at their boundaries (extreme points) by vertices corresponding to double intervals where a one-dimensional projection $P$ is chosen. The notion of ``maximal unions of adjacent vertices'' is therefore helpful in the formulation of the cluster expansion \eqref{eqclu1} and the weights $p(\mathcal{X)}$. We prove in Appendix \ref{AppC} that 
\begin{equation}
\label{p(G)}
p(\mathcal{X}):=\sum_{k=0}^{\infty }  \underset{[0,t_N]^{2k}} {\int} d\mu_k  (\underline{w})  \lambda( \underline{w})    \text{ }   \chi_{\mathcal{X} } (\underline{w})  \text{ F}(\underline{w})   \prod_{U \in \mathcal{U}(\mathcal{X})} h_U(\underline{w}),
\end{equation}
with
\begin{equation}
\label{hU}
 h_U(\underline{w}):=\langle \Pi (t_{m(U)}) \vert \mathcal{T}_S \Big( \underset{(i,B) \in U  }{\prod} \Big[ e^{-it_{i} \mathcal{L}_S} \big( \prod_{(t,r) \in  \underline{w} \cap \textbf{I}_i } (i G)(t,r) \big) e^{it_{i+1} \mathcal{L}_S} \Big]   \underset{(j,R) \in U  }{\prod} R(t_j) \Big) 1_S \rangle,
\end{equation}
 and where we have set  $\Pi(t_{-1}):= \vert \varphi  \rangle \langle \varphi \vert$ and  $R(t_{N}):=\textbf{L}(O)$.  The function $ \chi_{\mathcal{X}} (\underline{w})$ is equal to $1$ only  for pairings $\underline{w}$ that are compatible with the edges of  $\mathcal{X}$ (in the sense that the correlation lines of $\underline{w}$ follow the edges of $\mathcal{X}$). It takes the value zero otherwise.
 \vspace{2mm}












==> Section_Graph-3.tex <==

\section{ Rewriting $\mathcal{Z}^{t,0}$ as a sum over connected graphs}
\label{graphph}
 We  rewrite the Dyson expansion for  $\mathcal{Z}^{t,0}$  using graphs.  Our analysis contains three steps.\\
\vspace{1mm}

\noindent \textit{First step.} We discretize time on the Van Hove time scale and consider intervals $I_i:=[t_{i}, t_{i+1})$ with $t_{i+1}=t_{i} +\tau \lambda^{-2}(t_{i})$, $i=0,...,N-1$  and $t_0=0$.   We  introduce  four Feynman rules that correspond to the four possible contraction schemes  in the Dyson expansion \eqref{DD1'} and we associate a Feynman graph to each pairing  appearing under the integrals in  \eqref{DD1'}; see Paragraph \ref{Par1}.\\
 

\noindent \textit{Second step.}   We re-sum all  Feynman graphs  sharing  the same ``correlation properties''. What is meant  by  ``correlation properties'' will become apparent in subsection \ref{suba} below. In particular,  we re-sum all pairings  that have the property that any correlation  starting in one interval $I_i$  is also ending in $I_i$, $i=1,...,N$.   We then observe that these sums just correspond to the contribution of the product of the operators  
$\mathcal{Z}^{t_{i+1},t_{i}}$ to the Dyson series for $\mathcal{Z}^{t_N,0}$; see subsection \ref{suba}. \\
 

 \noindent \textit{Third step.} We use the decomposition \eqref{dec} of Lemma \ref{spectrum2}, in order to  rewrite  $ \langle \Psi(t) \vert O  \Psi(t) \rangle$ with the help of a cluster expansion. The one-dimensionality of the projections $P(t_i)$ plays an important role. Indeed, a product of operators 
 $A_1,..., A_n \in \mathcal{B} (\mathcal{B}(\mathcal{H}_S))$, when sandwiched  between two  projections $P(s_1)=\vert 1_S \rangle \langle \Pi(s_1) \vert $ and $P(s_2)=\vert 1_S \rangle \langle \Pi(s_2) \vert$, is equal to  
 \begin{equation*}
 P(s_1)A_1... A_n P(s_2)= P(s_2)  \text{ } \langle \Pi(s_2) \vert A_1... A_n \vert 1_s \rangle. 
\end{equation*}
Using this identity, we are able to assign a  scalar weight  to each element, $\mathcal{G}$, of a set of graphs or ``polymers'', denoted by $\mathbb{G}_{N}^{c}$. The set  $\mathbb{G}_{N}^{c}$ is constructed from the set of all possible pairings appearing in Wick's theorem;   see subsection \ref{secon}.


\subsection{Discretization of time, and Feynman rules }
\label{Par1}
We introduce a sequence $(t_i)_{i \geq 0}$ of times with the help of a recursion formula
\begin{equation}
\label{discr}
t_{i+1}=t_i +\tau \lambda^{-2}(t_i), \qquad t_0=0.
\end{equation}
We set
\begin{align}
\label{Ii}
I_{i}&:=\left[ t_{i}, t_{i+1}\right).
\end{align}
\input{curve}

\label{ff}
We introduce four  Feynman rules  corresponding to the four possible contractions displayed in \eqref{F2}:  
 %\input{lignetemps} 
\input{feynman}
corresponding to the ``operator-valued amplitudes''
\begin{align}
\label{fey1}
\textbf{(a)}&:=\lambda(u_i) \lambda(v_i)  f(u_i-v_i) \textbf{L}(iG(u_i)) \textbf{L}(iG(v_i)),  \\
\textbf{(b)}&:=\lambda(u_i) \lambda(v_i) f(u_i-v_i)  \textbf{L}(iG(u_i)) \textbf{R}(iG(v_i)),   \\
\textbf{(c)}&:=\lambda(u_i) \lambda(v_i) f(v_i-u_i)  \textbf{R}(iG(u_i)) \textbf{L}(iG(v_i)),   \\
\label{fey4}
\textbf{(d)}&:=\lambda(u_i) \lambda(v_i)  f(v_i-u_i) \textbf{R}(iG(u_i)) \textbf{R}(iG(v_i)).
\end{align}
The expressions (\ref{fey1})-(\ref{fey4}) can be read off directly from (\ref{F2}). To any operator 
$$ \lambda( \underline{u})  \lambda( \underline{v} )   \mathcal{T}_S \left[ \prod_{i=1}^{k}   \textbf{F}(u_{i},r_i ;v_{i},r'_i)  \right] $$
 in \eqref{DD1'} corresponds a unique Feynman graph,  constructed from the rules (\ref{fey1})-(\ref{fey4}), above. (Time ordering has to be carried out to determine the corresponding contribution to \eqref{DD1'}).   We are led to considering  graphs of a kind indicated in Figure 1. \input{graph2}

\newpage
\subsection{Re-summations}
\label{presum}
\subsubsection{Preliminary definitions}
We fix a natural number $N \in \mathbb{N}$. We associate an index $r$  To each  interval $I_i$, as defined in (\ref{Ii}), we associate an index $r$ that takes values $0$ or $1$. We set $\textbf{I}_i:=\left(I_{i},0;I_{i},1\right)$  and call $\textbf{I}_i$ a  double interval.  It corresponds to the picture
\begin{center}
\begin{tikzpicture}[scale=0.6]

\draw[-] (1,0) -- (2.5,0);
\draw[-,] (1,-3) -- (2.5,-3);

\draw[-,thick]  (1,-0.05) -- (1,0.05);
\draw[-,thick]  (2.5,-0.05) -- (2.5,0.05);

\draw[-,thick]  (1,-3.05) -- (1,-2.95);
\draw[-,thick]  (2.5,-3.05) -- (2.5,-2.95);


 \draw (1.05,0) node[below] {$t_{i}$};
 \draw (2.55,0) node[below] {$t_{i+1}$};
 \draw (1.05,-3) node[below] {$t_{i}$};
 \draw (2.55,-3) node[below] {$t_{i+1}$};
\end{tikzpicture}
\end{center}

\noindent The curved part from $t_N$ to $t_N$ in Figure \ref{M1} associated to the observable $O$ is  also considered to be a double interval and is denoted by  $\textbf{I}_{N}$.  There are two types of  double intervals in Figure \ref{M1}: $\textbf{I}_i$  is  either connected to  some  $\textbf{I}_j$ ($j \neq i$) by a correlation line; or any correlation that  starts  in  $\textbf{I}_i$ ends  in  $\textbf{I}_i$. In the first case, $\textbf{I}_i$ is said to be connected to $\textbf{I}_j$. In the second case, it is called isolated.   In Figure  \ref{M1}, $\textbf{I}_{3}$ and $\textbf{I}_{N}$ are  isolated, $\textbf{I}_{0}$ and $\textbf{I}_{1}$, $\textbf{I}_{1}$ and $\textbf{I}_{2}$,  $\textbf{I}_{2}$ and $\textbf{I}_{4}$,  $\textbf{I}_{4}$ and $\textbf{I}_{5}$ are connected.  Note that  $\textbf{I}_{N}$ is always isolated. 

\noindent {\red{End of corrections of JF, on Friday}}

 \begin{construction}
 \label{Con1}
  To each Feynman graph, we associate a new graph on the  vertex set of double intervals by drawing a line joining  the center of  $\textbf{I}_{i}$  to the center of  $\textbf{I}_{j}$ if   $\textbf{I}_{i}$ is connected to $\textbf{I}_{j}$ by at least one correlation line.
  \input{graph3}
\end{construction}
We erase the line $r=1$ as this information is not taken into account in the new graphs. To the Feynman graph of Figure \ref{M1} corresponds the graph
\input{graph4}

We denote by $\mathbb{F}_N$ the set of all possible graphs obtained  from all  possible pairings on $[0,t_N]$ following the construction \ref{Con1}.  $\mathbb{F}_N$ is finite.  A graph $\mathcal{G} =(\mathcal{V}(\mathcal{G}),\mathcal{L}(\mathcal{G})) \in \mathbb{F}_N$ has  a vertex set $\mathcal{V}(\mathcal{G})=\lbrace \textbf{I}_{0},...,\textbf{I}_{N} \rbrace$ and a set of lines $\mathcal{L}(\mathcal{G})$ that contains the lines joining the centers of the connected double intervals.  The construction of a graph $\mathcal{G} \in \mathbb{F}_N$ from a  given pairing (or its associated Feynman graph) is unique;  However, many pairings may give rise to the same graph $\mathcal{G}$. We then say that a  pairing $\underline{w}$  is \textit{compatible} with  $\mathcal{G}$ if its corresponding Feynman graph gives rise to the graph $\mathcal{G}$ within the  construction \ref{Con1}. We also introduce  the function $\mathds{1}_{\mathcal{G}}$   defined on the set of all possible pairings by
\begin{equation}
\mathds{1}_{\mathcal{G}}(\underline{w}):=\left\{ \begin{array}{cc}  1 & \text{ if } \underline{w} \text{ is compatible with } \mathcal{G},\\0 & \text{ otherwise}. \end{array} \right.
\end{equation}
Moreover,
\begin{equation}
\label{unic}
\sum_{\mathcal{G} \in  \mathbb{F}_N} \mathds{1}_{\mathcal{G}}(\underline{w})=1
\end{equation}
for any fixed pairing $\underline{w}$. We now re-sum over all pairings giving rise to the same graph $\mathcal{G} \in \mathbb{F}_N$.   Plugging \eqref{unic} into (\ref{DD1'}), we get that
\begin{equation}
\label{DD12}
 \mathcal{Z}^{t_N,0}(O)  = \sum_{\mathcal{G} \in \mathbb{F}_N}  \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O)  
\end{equation}
where
\begin{equation}
\label{DD13}
 \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O)    := \sum_{k=0}^{\infty}  \underset{[0,t]^{2k}}{\int} d\mu_k(\underline{w})  \lambda( \underline{w})  \text{ } \mathds{1}_{\mathcal{G}}(\underline{w}) \mathcal{T}_S \left[     \textbf{F}( \underline{w})  \right] \left[ O(t_N) \right].
\end{equation}
 

\subsubsection{  Re-summing  pairs inside isolated intervals }
\label{suba}

Let $\mathcal{G} \in \mathbb{F}_N$. We assume that  $\mathcal{G} $ contains  at least one isolated  interval   $\textbf{I}_{i_0}$,  $i_0 \neq N$. The function $ \mathds{1}_{\mathcal{G}}(\underline{w}) $ selects the  pairings $\underline{w}$ that have the property  that any time $u_i \in \textbf{I}_{i_0}$ is   contracted with  a  time $v_i \in \textbf{I}_{i_0}$. We  re-sum  over all the  pairs   $(u_i,r_i;v_i,r'_i)$ with  $u_i,v_i \in \textbf{I}_{i_0}$.  Exchange of sums and integrals  are  carried out without further justifications since the Dyson series converge absolutely;  see $\eqref{labound}$. For any disjoint union of intervals  $J=I_1 \cup \text{ }...\text{ } \cup I_l \subset \mathbb{R}_+$, we  introduce the measure
\begin{equation}
\label{mu2}
d\mu_{k,J} (\underline{w}):= \sum_{\underline{r},\underline{r}' \in \lbrace 0,1 \rbrace^{k}}  \text{ } d \underline{u} d \underline{v}  \text{ }  \chi(u_1<...<u_k)  \text{ } \prod_{i=1}^{k} ( \chi(u_i<v_i)  \chi(u_i,v_i \in J)).
\end{equation}
We  introduce the functions $\mathds{1}_{\mathcal{G}, J ,m}$, $m \in \mathbb{N} \cup \{0\}$,  defined on the set of all possible pairings  by
\begin{equation}
\mathds{1}_{\mathcal{G}, J ,m}(\underline{w}):=\left\{ \begin{array}{ll}  1 & \text{ if } \underline{w} \text{ is compatible with }   \mathcal{G} \text{ and  has exactly }  m  \text{ pairs  in }   J, \\0 & \text{ otherwise}. \end{array} \right. 
\end{equation}

\noindent
For every tuple $\underline{w}$ of $k$ pairs, 
\begin{equation}
\label{1G}
\mathds{1}_{\mathcal{G}}(\underline{w})=  \sum_{m=0}^{k} \mathds{1}_{\mathcal{G}, J,m}(\underline{w})
  \end{equation}
for all $\mathcal{G} \in \mathbb{F}_N$ and for all $J \subset \mathcal{V}(\mathcal{G})$. We plug (\ref{1G})  and (\ref{mu2})  into (\ref{DD13}) with $J= \textbf{I}_{i_0}$, and  we get that
\begin{equation}
\label{DD14}
\begin{split}
 \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O)=\sum_{k=0}^{\infty}  \sum_{m=0}^{k}  \underset{[0,t_N]^{2k}}{\int} d\mu_k (\underline{w})  \lambda( \underline{w})    \text{ } \mathds{1}_{\mathcal{G}, \textbf{I}_{i_0} ,m}(\underline{w}) \mathcal{T}_S \left[ \prod_{i=1}^{k}   \text{ }  {\bf{F}}(\underline{w})  \right] \left[ O(t_N) \right].
\end{split}
\end{equation}
If  $\mathds{1}_{\mathcal{G}, \textbf{I}_{i_0} ,m}(\underline{w}) =1$ for some $m \in \mathbb{N}$, there are two unique  tuples $\underline{\tilde{w}}$ and $\underline{\hat{w}}$  with  $\underline{w}=\underline{\tilde{w}} \cup \underline{\hat{w}}$  such  that all times in $\underline{\hat{w}}$  lie in $\textbf{I}_{i_0}$ and  no time in   $\underline{\tilde{w}}$ lies in $\textbf{I}_{i_0}$. Up to a change of variables,  we can cut the integral in \eqref{DD14} into two distinct integrals. Exchanging the sum over $k$ with the sum over $m$, we  finally get that 
\begin{equation*}
%\label{DD16}
 \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O)=\sum_{k=0}^{\infty}  \underset{[0,t_N]^{2k}}{\int} d\mu_{k}  (\underline{\tilde{w}})  \lambda( \underline{\tilde{w}})  \text{ }  \mathds{1}_{\mathcal{G} \setminus \textbf{I}_{i_0} } ( \underline{\tilde{w}})\\
 \mathcal{T}_S \Big(    \textbf{F}( \underline{\tilde{w}})  \sum_{m=0}^{\infty}  \underset{ I_{i_0}}{\int} d\mu_m (\underline{\hat{w}})  \lambda( \underline{\hat{w}})    \mathcal{T}_S \left[   \textbf{F}( \underline{\hat{w}})  \right] \Big) \left[ O(t_N) \right].
\end{equation*}
We recognize the operator $e^{i t_{i_{0}} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+1},t_{i_0}}e^{-i t_{i_0+1} \mathcal{L}_S}$  inside the parentheses; see \eqref{DD1'}.  Note that $\mathds{1}_{\mathcal{G} \setminus \textbf{I}_{i_0} } $  selects only the pairings compatible with $\mathcal{G}$ with no pairs in $\textbf{I}_{i_0}$. Repeating this procedure again for each isolated  interval,  we get the lemma.

\begin{lemma} 
\label{coiso}
Let $\mathcal{G} \in  \mathbb{F}_N$  with isolated  intervals $\textbf{I}_{i_0},...,\textbf{I}_{i_m}$, $i_0,...,i_m \neq N$. Then
\begin{equation}
\label{DDtt}
\begin{split}
 \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O) & =\sum_{k=0}^{\infty}      \underset{[0,t_N]^{2k}}{\int} d\mu_{k} (\underline{w})  \lambda( \underline{w})    \text{ }  \mathds{1}_{\mathcal{G} \setminus (\textbf{I}_{i_0}  \cup...\cup \textbf{I}_{i_m}) } (\underline{w}) \\
 &\mathcal{T}_S \left(      \textbf{F}( \underline{w} ) \text{ }  e^{i t_{i_{0}} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+1},t_{i_0}}e^{-i t_{i_0+1} \mathcal{L}_S}  \text{ } ... \text{ }e^{i t_{i_{m}} \mathcal{L}_S}\mathcal{Z}^{t_{i_m+1},t_{i_m}}e^{-i t_{i_m+1} \mathcal{L}_S} \right) \left[ O(t_N) \right] 
 \end{split}
\end{equation}
for all $O \in \mathcal{B}(\mathcal{H}_S)$.
\end{lemma}
\vspace{2mm}

\subsection{Connected graphs and cluster expansion}
\label{secon}
\subsubsection{Construction of the set $\mathbb{G}_N$}
We use  that 
\begin{equation}
 \label{dec2}
 \mathcal{Z}^{t_{i+1},t_{i}}= P(t_i)+R(t_i)
 \end{equation}
(see Lemma \ref{spectrum2})  to  rewrite $\langle \Psi(t_N)  \vert (O  \otimes 1)   \Psi(t_N) \rangle$  with a polymer expansion. Remark that
\begin{equation*}
e^{i t_{i_{0}} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+1},t_{i_0}}e^{-i t_{i_0+1} \mathcal{L}_S} e^{i t_{i_{0}+1} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+2},t_{i_0+1}} e^{-i t_{i_0+2} \mathcal{L}_S}
=e^{i t_{i_{0}} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+1},t_{i_0}} \mathcal{Z}^{t_{i_0+2},t_{i_0+1}} e^{-i t_{i_0+2}  \mathcal{L}_S}
\end{equation*}
and that
\begin{equation*}
e^{i t_{N-1} \mathcal{L}_S} \mathcal{Z}^{t_{N},t_{N-1}} e^{-i t_{N} \mathcal{L}_S} O(t_N)=e^{i t_{N-1} \mathcal{L}_S} \mathcal{Z}^{t_{N},t_{N-1}} O.
\end{equation*}
This shows that the operators $e^{it_j \mathcal{L}_S}$  cancel each other in the product inside the parentheses in \eqref{DDtt} if they are not located at the extremities of  a union of adjacent isolated  intervals. We   extend   the time ordering operator $\mathcal{T}_S$   in such a way that  $\mathcal{T}_S$ orders $e^{i t_{i_{l}} \mathcal{L}_S}$ on the right of $e^{-i t_{i_{l}} \mathcal{L}_S}$  and $e^{-i t_{i_{l}+1} \mathcal{L}_S}$ on the right of  $\mathcal{Z}^{t_{i_l+1},t_{i_l}}$. We   then rewrite
\begin{equation}
\label{DDt}
\begin{split}
 \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O)=\sum_{k=0}^{\infty} &    \underset{[0,t_N]^{2k} }{\int} d\mu_{k} (\underline{w})  \lambda( \underline{w})    \text{ }  \mathds{1}_{\mathcal{G} \setminus (\textbf{I}_{i_0}  \cup...\cup \textbf{I}_{i_m}) } (\underline{w}) \\
 &\mathcal{T}_S \Big(    \big( \prod_{l=0}^{m}  e^{-i t_{i_{l}+1} \mathcal{L}_S}  \big)    \textbf{F}( \underline{w} )   \big( \prod_{l=0}^{m}  e^{i t_{i_{l}} \mathcal{L}_S}  \big) \mathcal{Z}^{t_{i_0+1},t_{i_0}} \text{ } ... \text{ } \mathcal{Z}^{t_{i_m+1},t_{i_m}}  \Big) [ O(t_N) ]
 \end{split}
\end{equation} 

\noindent We  construct a new set of graphs  by  inserting  (\ref{dec2}) into (\ref{DDt})  for each $\mathcal{G} \in \mathbb{F}_N$.  If $\mathcal{V}(\mathcal{G})$ contains  $m+1$ isolated intervals different from $I_{N+1}$, we get  $2^{m+1}$ terms of the form
\begin{equation}
\label{DDt2}
\begin{split}
\sum_{k=0}^{\infty}  &  \underset{[0,t_N]^{2k}  }{\int} d\mu_{k} (\underline{w})  \lambda( \underline{w})    \text{ }  \mathds{1}_{\mathcal{G} \setminus (\textbf{I}_{i_0}  \cup...\cup \textbf{I}_{i_m}) } (\underline{w}) \\
 &\mathcal{T}_S \Big(    \big( \prod_{l=0}^{m}  e^{-i t_{i_{l}+1} \mathcal{L}_S}  \big)    \textbf{F}( \underline{w} )   \big( \prod_{l=0}^{m}  e^{i t_{i_{l}} \mathcal{L}_S}  \big) P(t_{i_0}) R(t_{i_1})   ... \text{ } R(t_{i_m})   \Big) \left[ O(t_N)  \right] .
 \end{split}
\end{equation}
We associate a graph to each of these $2^{m+1}$ terms. 
\vspace{2mm}

\noindent
\begin{construction} 
Let $\mathcal{G}$ be a graph in $\mathbb{F}_N$ with $m+1$ isolated vertices distinct from $\textbf{I}_N$. Using the decomposition \eqref{dec2}, we construct $2^{m+1}$ new graphs by following the procedure:
\begin{itemize}
\item If   $\textbf{I}_{i}$  carries a projection $P(t_{i})$, we erase $\textbf{I}_{i}$ from the vertex set of  $\mathcal{G}$.
\item If  $\textbf{I}_{i}$ carries  a perturbation $R(t_{i})$, we let $\textbf{I}_{i}$  in the vertex set of the graph, and mark it with the symbol
\begin{center}
\begin{tikzpicture}[scale=0.8]
\draw[ snake=zigzag]  (0.0,0.0) -- (2,0.0);
\fill (1,0) circle (0.1cm);
\end{tikzpicture}
\end{center}
\item  $\textbf{I}_{N}$ is  kept in the vertex set of the new graph and is marked  in bold.
\end{itemize}
We carry out  this construction for all  graphs in $\mathbb{F}_N$. We obtain a new finite set of graphs  that we denote by $\mathbb{G}_N$. A graph  $\mathcal{G}=(\mathcal{V}(\mathcal{G}),\mathcal{L}(\mathcal{G})) \in \mathbb{G}_N$ has a vertex set $\mathcal{V}(\mathcal{G})$ contained in $\lbrace \textbf{I}_0,..., \textbf{I}_{N} \rbrace$ and a set of lines   $\mathcal{L}(\mathcal{G})$. 
\end{construction}
\vspace{2mm}

\noindent As an example, it is easy to see that  we construct two new graphs from  the  figure \ref{bel2}.
\input{graph6}

  The vertex set $\mathcal{V}(\mathcal{G})$   of a graph $\mathcal{G}$ can be  divided into two disjoint subsets: the set of bound intervals, that we denote by $\mathcal{B}(\mathcal{G})$, and the set  of $R$-intervals (that carry a perturbation $R$), denoted by $\mathcal{R}(\mathcal{G})$.  A line $\mathscr{L}=(\textbf{I}_i,\textbf{I}_j) \in \mathcal{L}(\mathcal{G})$  $(i<j)$  binds  two intervals $\textbf{I}_i, \textbf{I}_j \in \mathcal{B}(\mathcal{G})$.  As in \eqref{DD12}, we  have that
 \begin{equation}
\label{DD12'}
 \mathcal{Z}^{t_N,0}(O)= \sum_{\mathcal{G} \in \mathbb{G}_N}  \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O),
 \end{equation}
but  the effective dynamics associated  to a graph $\mathcal{G} \in \mathbb{G}_N$ is now given by
\begin{equation}
\label{DDt2}
\begin{split}
 \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O): =\sum_{k=0}^{\infty}  &  \underset{[0,t_N]^{2k}  }{\int} d\mu_{k} (\underline{w})  \lambda( \underline{w})    \text{ }  \mathds{1}_{(\mathcal{B}(\mathcal{G}),\mathcal{L}(\mathcal{G})) } (\underline{w}) \\
 &\mathcal{T}_S \Big(    \big( \prod_{l,   \textbf{I}_l \notin \mathcal{B}(\mathcal{G})}  e^{-i t_{l+1} \mathcal{L}_S} e^{i t_{l} \mathcal{L}_S} \big)    \textbf{F}( \underline{w} )    \prod_{i, \textbf{I}_i \in \mathcal{R}(\mathcal{G})}   R(t_i)   \prod_{j, \textbf{I}_j \notin \mathcal{V}(\mathcal{G})}   P(t_j) \Big) [ \mathds{1}_S ],
 \end{split}
\end{equation}
where we have  set  $R(t_{N+1})=\textbf{L}(O)$.
We now decompose every  graph $\mathcal{G} \in \mathbb{G}_N$ into a disjoint union of connected subgraphs. The set of \textit{connected  graphs}  $\mathbb{G}^{c}_{N}$ is the polymer set of our cluster expansion. 
 
 \subsubsection{Construction of the set $\mathbb{G}_{N}^{c}$}
 A line $\mathscr{L} \in \mathcal{L}(\mathcal{G})$ is  represented by the drawing
\begin{center}
\begin{tikzpicture}[scale=0.5]

\fill (3.5,0) circle (0.1cm);
\fill (8.5,0) circle (0.1cm);


\draw[-] (3.5,0) -- (6, 1.0); 
\draw[-] (6,1) -- (8.5, 0.0);

\end{tikzpicture}
\end{center}
\noindent An \textit{adjacent edge} is an edge joining the center of two adjacent  intervals. There are 3 possible adjacent edges:
\begin{center}
\begin{tikzpicture}[scale=0.5]

\fill (3.5,0) circle (0.1cm);
\fill (6.5,0) circle (0.1cm);

\draw[-] (3.5,0) -- (6.5, 0.0); 

\fill (10.5,0) circle (0.1cm);
\fill (13.5,0) circle (0.1cm);
\draw[ -] (10.5,0) -- (12, 0.0); 
\draw[ snake=zigzag] (12,0) -- (13.5, 0.0); 


\fill (15.5,0) circle (0.1cm);
\fill (18.5,0) circle (0.1cm);
\draw[ snake=zigzag] (15.5,0) -- (17, 0.0); 
\draw[ -] (17,0) -- (18.5, 0.0); 

  
\end{tikzpicture}
\end{center}

A \textit{path}  from $\textbf{I}_{i}$ to $\textbf{I}_{j}$ is naturally defined as a non-broken succession of  lines and adjacent edges from the center of $\textbf{I}_i$ to the center of $\textbf{I}_j$; see the figure below. We say that a graph $\mathcal{G} \in \mathbb{G}_{N}$ is \textit{connected} if  there is a path joining  $\textbf{I}_i$ to  $\textbf{I}_j$ for all  $\textbf{I}_i \neq \textbf{I}_j \in \mathcal{V}(\mathcal{G})$. The set of \textit{connected graphs} is denoted by $\mathbb{G}^{c}_{N}$.
 \begin{center}
\begin{tikzpicture}[scale=0.5]

\fill (3.5,0) circle (0.1cm);
\fill (6.5,0) circle (0.1cm);
\fill (-1,0) circle (0.1cm);

 \draw (-1,0) node[below] {$\textbf{I}_{t_1}$};
  \draw (12.5,0) node[below] {$\textbf{I}_{t_2}$};
  
\draw[-] (6.5,0) -- (9.5, 0.0); 
\draw[-] (3.5,0) -- (5, 1.0); 
\draw[-] (5,1.0) -- (6.5, 0.0); 

\fill (9.5,0) circle (0.1cm);
\fill (12.5,0) circle (0.1cm);
\draw[ snake=zigzag] (10.5,0) -- (12.5, 0.0); 
\draw[ -] (9.5,0) -- (10.5, 0.0); 

\draw[ -] (-1,0) -- (1.25, 1.0); 
\draw[ -] (1.25, 1.0) -- (3.5, 0.0); 

 \draw (6.5,-1.5) node[below] {\footnotesize A path from $\textbf{I}_{t_1}$ to  $\textbf{I}_{t_2}$};

\end{tikzpicture}
\end{center}
\input{graph7}
\vspace{2mm}

It is  useful to introduce the notion of \textit{maximal union of adjacent vertices }.  We say that a disjoint union   $U=\cup_i  \text{ } \textbf{I}_{i} \subset \mathcal{V}(\mathcal{G})$ of  adjacent  vertices  is  a maximal union of adjacent vertices  if,  for any $\textbf{I}_{i}, \textbf{I}_{j} \in U$,  there is an adjacent path joining $\textbf{I}_{i}$ to $\textbf{I}_{j}$,  and if $U$ is the biggest set in $\mathcal{V}(\mathcal{G})$ in the sense of the inclusion having this property.  We denote by  $\mathcal{U}(\mathcal{G})$ the set of maximal unions of adjacent vertices  of  $\mathcal{G}$.  Maximal unions of adjacent vertices are  surrounded at their  extremities by  one-dimensional projections $P$, and this is the reason why we  need them to write the polymer expansion.  


\subsubsection{The polymer expansion}
Before writing our polymer expansion for the effective dynamics $\mathcal{Z}^{t_N,0}$, we introduce three further useful notations. We define
\begin{align}
\label{mmm}
m(A)&:= \min \{ i \mid  \textbf{I}_{i} \in A \}-1,\\
\label{MMM}
M(A)&:=\max \{ i \mid  \textbf{I}_{i} \in A \}+1
\end{align}
for all sets $A \subset \mathcal{V}(\mathcal{G})$ and 
\begin{equation}
\mbox{dist} \left(\mathcal{G}, \mathcal{G}' \right)=\underset{\textbf{I}_{i} \in \mathcal{V}(\mathcal{G}), \text{ } \textbf{I}_{j} \in \mathcal{V}(\mathcal{G'})}{\min}  (\vert i-j  \vert-1) 
\end{equation}
for all  $\mathcal{G}$, $\mathcal{G'} \in   \mathbb{G}_N$. Two  adjacent graphs have a distance equal to $0$. It is clear that any graph $\mathcal{G} \in \mathbb{G}_N$ possesses a unique decomposition into connected subgraphs, separated each other by a distance bigger or equal to one.  This remarks leads to the lemma


\begin{lemma}
\label{facto}
Let $\mathcal{G} =\mathcal{G}_1 \vee ... \vee \mathcal{G}_q  \in \mathbb{G}_N$, with $\mathcal{G}_1,...,\mathcal{G}_q \in  \mathbb{G}^{c}_{N}$  and $ \text{dist}(\mathcal{G}_i,\mathcal{G}_j) \geq 1$ for all $ i\neq j$.  Then
\begin{equation}
\label{prodd}
\langle \varphi  \vert \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O)  \varphi \rangle  =p(\mathcal{G}_1)\text{ }... \text{ }p(\mathcal{G}_q)
\end{equation}

\noindent where $p: \mathbb{G}_{N}^{c} \rightarrow \mathbb{C}$ is  defined by
\begin{equation}
\label{p(G)}
p(\mathcal{G}):=\sum_{k=0}^{\infty }  \underset{[0,t_N]^{2k}} {\int} d\mu_k  (\underline{w})  \lambda( \underline{w})    \text{ }   \mathds{1}_{(\mathcal{B}(\mathcal{G}),\mathcal{L}(\mathcal{G})) } (\underline{w})  \text{ F}(\underline{w})   \prod_{U \in \mathcal{U}(\mathcal{G})} h(U,\underline{w})
\end{equation}
and where we have set
\begin{equation*}
 h(U ,\underline{w}):=\langle \Pi (t_{m(U)}) \vert \mathcal{T}_S \Big( \underset{i, \textbf{I}_i \in U \cap \mathcal{B}(\mathcal{G}) }{\prod} \Big[ e^{-it_{i} \mathcal{L}_S} \big( \prod_{(t,r) \in  \underline{w} \cap \textbf{I}_i } (i G)(t,r) \big) e^{it_{i+1} \mathcal{L}_S} \Big]   \underset{j, \textbf{I}_j \in U \cap \mathcal{R}(\mathcal{G}) }{\prod} R(t_j) \Big) 1_S \rangle,
\end{equation*}
\begin{equation*}
\Pi(t_{-1}):= \vert \varphi  \rangle \langle \varphi \vert  \qquad   \text{ and } \qquad  R(t_{N}):=\textbf{L}(O).
\end{equation*}
 \end{lemma}
\vspace{2mm}

\noindent  The proof of Lemma \ref{facto} is carried out in the appendix.   Lemma \ref{facto}  readily  implies   that the  expectation value $\langle \Psi(t_N) \vert  O    \Psi(t_N) \rangle$ can be rewritten as a cluster expansion over the polymer set $\mathbb{G}^{c}_{N}$.



\begin{proposition}
\label{clustt}
\begin{align}
\label{eqclu1}
\langle \Psi (t_N) \vert (O  \otimes 1)   \Psi(t_N) \rangle&=  \sum_{q=1}^{N} \frac{1}{q!} \underset{\text{dist}(\mathcal{G}_i,\mathcal{G}_j) \geq 1, \text{ } \exists i_0, \text{ }\textbf{I}_{N} \in \mathcal{V}( \mathcal{G}_{i_0})}{\underset{\mathcal{G}_1,...,\mathcal{G}_q \in \mathbb{G}^{c}_{N}}{\sum}}   p\left(\mathcal{G}_1\right)...\text{ }p\left(\mathcal{G}_q\right), \\
\label{eqclu2}
\langle   \Psi (t_N) \vert   \Psi (t_N) \rangle&=   1 +  \sum_{q=1}^{N} \frac{1}{q!} \underset{\text{dist}(\mathcal{G}_i,\mathcal{G}_j) \geq 1,  \text{ }\textbf{I}_{N} \notin \mathcal{V}( \mathcal{G}_{i}) } {\underset{\mathcal{G}_1,...,\mathcal{G}_q \in \mathbb{G}^{c}_{N}}{\sum}}   \text{ } \text{ } p\left(\mathcal{G}_1\right)...\text{ }p\left(\mathcal{G}_q\right).
\end{align}
\end{proposition}
\vspace{4mm}


\begin{remark}The factor $q!$ comes from the permutation of the graphs  in $\mathbb{G}^{c}_{N}$ . The sum over $q$  is finite and ends  if  it is  not possible to find  $\mathcal{G}_1,...,\mathcal{G}_q \in \mathbb{G}^{c}_{N}$ such that  $\mathcal{G} =\mathcal{G}_1 \vee ... \vee \mathcal{G}_m  \in \mathbb{G}_N$, with $\mathcal{G}_1,...,\mathcal{G}_m \in  \mathbb{G}^{c}_{N}$  and $ \text{dist}(\mathcal{G}_i,\mathcal{G}_j) \geq 1$ for all $ i\neq j$.
\end{remark}

















==> Section_Graph_3.tex <==

\section{ Rewriting $\mathcal{Z}^{t,0}$ as a sum over connected graphs}
\label{graphph}
 We  rewrite the Dyson expansion for  $\mathcal{Z}^{t,0}$  using graphs.  Our analysis contains three steps.\\
\vspace{1mm}

\noindent \textit{First step.} We discretize time on the Van Hove time scale and consider intervals $I_i:=[t_{i}, t_{i+1})$ with $t_{i+1}=t_{i} +\tau \lambda^{-2}(t_{i})$, $i=0,...,N-1$  and $t_0=0$.   We  introduce  four Feynman rules that correspond to the four possible contraction schemes  in the Dyson expansion \eqref{DD1'} and we associate a Feynman graph to each pairing  appearing under the integrals in  \eqref{DD1'}; see Paragraph \ref{Par1}.\\
 

\noindent \textit{Second step.}   We re-sum all  Feynman graphs  sharing  the same "correlation properties". What is meant  by  "correlation properties"  will become clear in Paragraph \ref{suba} below. In particular,  we re-sum all pairings  that have the property that any correlation  starting in one interval $I_i$  is also ending in $I_i$, $i=1,...,N$.   We then  recognize the contribution of  the operators   $\mathcal{Z}^{t_{i+1},t_{i}}$ to  the Dyson series; see Paragraph \ref{suba}. \\
 

 \noindent \textit{Third step.} We use the decomposition \eqref{dec} of Lemma \ref{spectrum2}  and  rewrite  $ \langle \Psi(t) \vert O  \Psi(t) \rangle$ with a cluster expansion. The one-dimensionality of the projections $P(t_i)$ plays an important role. Indeed, a product of operators $A_1,..., A_n \in \mathcal{B} (\mathcal{B}(\mathcal{H}_S))$ sandwiched  between two  projections $P(s_1)=\vert 1_S \rangle \langle \Pi(s_1) \vert $ and $P(s_2)=\vert 1_S \rangle \langle \Pi(s_2) \vert$ is equal to  
 \begin{equation*}
 P(s_1)A_1... A_n P(s_2)= P(s_2)  \text{ } \langle \Pi(s_2) \vert A_1... A_n \vert 1_s \rangle. 
\end{equation*}
We use this property to associate a  scalar weight  to each element $\mathcal{G}$ of a polymer set of graphs, $\mathbb{G}_{N}^{c}$. The  polymer set  $\mathbb{G}_{N}^{c}$ is directly constructed from the set of all possible pairings;   see Paragraph \ref{secon}.


\subsection{Time discretization and Feynman rules }
\label{Par1}
We introduce the sequence $(t_i)_{i \geq 0}$, defined by
\begin{equation}
\label{discr}
t_{i+1}=t_i +\tau \lambda^{-2}(t_i), \qquad t_0=0.
\end{equation}
We set
\begin{align}
\label{lambda}
\lambda_i&:=\lambda(t_i),\\
\label{Ii}
I_{i}&:=\left[ t_{i}, t_{i+1}\right).
\end{align}
\input{curve}

\label{ff}
We introduce four  Feynman rules  corresponding to the four possible contractions given in \eqref{F2}:  
 %\input{lignetemps} 
\input{feynman}
with the contributions
\begin{align}
\label{fey1}
\textbf{(a)}&:=\lambda(u_i) \lambda(v_i)  f(u_i-v_i) \textbf{L}(iG(u_i)) \textbf{L}(iG(v_i)),  \\
\textbf{(b)}&:=\lambda(u_i) \lambda(v_i) f(u_i-v_i)  \textbf{L}(iG(u_i)) \textbf{R}(iG(v_i)),   \\
\textbf{(c)}&:=\lambda(u_i) \lambda(v_i) f(v_i-u_i)  \textbf{R}(iG(u_i)) \textbf{L}(iG(v_i)),   \\
\label{fey4}
\textbf{(d)}&:=\lambda(u_i) \lambda(v_i)  f(v_i-u_i) \textbf{R}(iG(u_i)) \textbf{R}(iG(v_i)).
\end{align}
The rules (\ref{fey1})-(\ref{fey4}) are directly deduced from (\ref{F2}). To any operator 
$$ \lambda( \underline{u})  \lambda( \underline{v} )   \mathcal{T}_S \left[ \prod_{i=1}^{k}   \textbf{F}(u_{i},r_i ;v_{i},r'_i)  \right] $$
 in \eqref{DD1'} corresponds a unique Feynman graph,  constructed from the rules (\ref{fey1})-(\ref{fey4}) above. Time ordering has to be carried out to compute its contribution to \eqref{DD1'}.   We are led to consider  graphs of the form
\input{graph2}


\subsection{Re-summing}
\label{presum}
\subsubsection{Preliminary definitions}
We now fix $N \in \mathbb{N}$. We associate an index $r$  to each  interval $I_i$ as defined in (\ref{Ii}) that takes the value $0$ or $1$. We set $\textbf{I}_i:=\left(I_{i},0;I_{i},1\right)$  and call $\textbf{I}_i$ a  double interval.  It corresponds to the picture
\begin{center}
\begin{tikzpicture}[scale=0.6]

\draw[-] (1,0) -- (2.5,0);
\draw[-,] (1,-3) -- (2.5,-3);

\draw[-,thick]  (1,-0.05) -- (1,0.05);
\draw[-,thick]  (2.5,-0.05) -- (2.5,0.05);

\draw[-,thick]  (1,-3.05) -- (1,-2.95);
\draw[-,thick]  (2.5,-3.05) -- (2.5,-2.95);


 \draw (1.05,0) node[below] {$t_{i}$};
 \draw (2.55,0) node[below] {$t_{i+1}$};
 \draw (1.05,-3) node[below] {$t_{i}$};
 \draw (2.55,-3) node[below] {$t_{i+1}$};
\end{tikzpicture}
\end{center}

\noindent The curved part from $t_N$ to $t_N$ in Figure \ref{M1} associated to the observable $O$ is  also considered as a double interval and is denoted by  $\textbf{I}_{N}$.  There are two types of  double intervals in Figure \ref{M1}: $\textbf{I}_i$  is  either connected to  some  $\textbf{I}_j$ ($j \neq i$) by a correlation line; or any correlation that  starts  in  $\textbf{I}_i$ ends  in  $\textbf{I}_i$. In the first case, $\textbf{I}_i$ is said to be connected to $\textbf{I}_j$. In the second case, it is called isolated.   In Figure  \ref{M1}, $\textbf{I}_{3}$ and $\textbf{I}_{N}$ are  isolated, $\textbf{I}_{0}$ and $\textbf{I}_{1}$, $\textbf{I}_{1}$ and $\textbf{I}_{2}$,  $\textbf{I}_{2}$ and $\textbf{I}_{4}$,  $\textbf{I}_{4}$ and $\textbf{I}_{5}$ are connected.  Note that  $\textbf{I}_{N}$ is always isolated. 

 \begin{construction}
 \label{Con1}
  To each Feynman graph, we associate a new graph on the  vertex set of double intervals by drawing a line joining  the center of  $\textbf{I}_{i}$  to the center of  $\textbf{I}_{j}$ if   $\textbf{I}_{i}$ is connected to $\textbf{I}_{j}$ by at least one correlation line.
  \input{graph3}
\end{construction}
We erase the line $r=1$ as this information is not taken into account in the new graphs. To the Feynman graph of Figure \ref{M1} corresponds the graph
\input{graph4}

We denote by $\mathbb{F}_N$ the set of all possible graphs obtained  from all  possible pairings on $[0,t_N]$ following the construction \ref{Con1}.  $\mathbb{F}_N$ is finite.  A graph $\mathcal{G} =(\mathcal{V}(\mathcal{G}),\mathcal{L}(\mathcal{G})) \in \mathbb{F}_N$ has  a vertex set $\mathcal{V}(\mathcal{G})=\lbrace \textbf{I}_{0},...,\textbf{I}_{N} \rbrace$ and a set of lines $\mathcal{L}(\mathcal{G})$ that contains the lines joining the centers of the connected double intervals.  The construction of a graph $\mathcal{G} \in \mathbb{F}_N$ from a  given pairing (or its associated Feynman graph) is unique;  However, many pairings may give rise to the same graph $\mathcal{G}$. We then say that a  pairing $\underline{w}$  is \textit{compatible} with  $\mathcal{G}$ if its corresponding Feynman graph gives rise to the graph $\mathcal{G}$ within the  construction \ref{Con1}. We also introduce  the function $\mathds{1}_{\mathcal{G}}$   defined on the set of all possible pairings by
\begin{equation}
\mathds{1}_{\mathcal{G}}(\underline{w}):=\left\{ \begin{array}{cc}  1 & \text{ if } \underline{w} \text{ is compatible with } \mathcal{G},\\0 & \text{ otherwise}. \end{array} \right.
\end{equation}
Moreover,
\begin{equation}
\label{unic}
\sum_{\mathcal{G} \in  \mathbb{F}_N} \mathds{1}_{\mathcal{G}}(\underline{w})=1
\end{equation}
for any fixed pairing $\underline{w}$. We now re-sum over all pairings giving rise to the same graph $\mathcal{G} \in \mathbb{F}_N$.   Plugging \eqref{unic} into (\ref{DD1'}), we get that
\begin{equation}
\label{DD12}
 \mathcal{Z}^{t_N,0}(O)  = \sum_{\mathcal{G} \in \mathbb{F}_N}  \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O)  
\end{equation}
where
\begin{equation}
\label{DD13}
 \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O)    := \sum_{k=0}^{\infty}  \underset{[0,t]^{2k}}{\int} d\mu_k(\underline{w})  \lambda( \underline{w})  \text{ } \mathds{1}_{\mathcal{G}}(\underline{w}) \mathcal{T}_S \left[     \textbf{F}( \underline{w})  \right] \left[ O_{t_N} \right].
\end{equation}
 

\subsubsection{  Re-summing  pairs inside isolated intervals }
\label{suba}

Let $\mathcal{G} \in \mathbb{F}_N$. We assume that  $\mathcal{G} $ contains  at least one isolated  interval   $\textbf{I}_{i_0}$,  $i_0 \neq N$. The function $ \mathds{1}_{\mathcal{G}}(\underline{w}) $ selects the  pairings $\underline{w}$ that have the property  that any time $u_i \in \textbf{I}_{i_0}$ is   contracted with  a  time $v_i \in \textbf{I}_{i_0}$. We  re-sum  over all the  pairs   $(u_i,r_i;v_i,r'_i)$ with  $u_i,v_i \in \textbf{I}_{i_0}$.  Exchange of sums and integrals  are  carried out without further justifications since the Dyson series converge absolutely;  see $\eqref{labound}$. For any disjoint union of intervals  $J=I_1 \cup \text{ }...\text{ } \cup I_l \subset \mathbb{R}_+$, we  introduce the measure
\begin{equation}
\label{mu2}
d\mu_{k,J} (\underline{w}):= \sum_{\underline{r},\underline{r}' \in \lbrace 0,1 \rbrace^{k}}  \text{ } d \underline{u} d \underline{v}  \text{ }  \chi(u_1<...<u_k)  \text{ } \prod_{i=1}^{k} ( \chi(u_i<v_i)  \chi(u_i,v_i \in J)).
\end{equation}
We  introduce the functions $\mathds{1}_{\mathcal{G}, J ,m}$, $m \in \mathbb{N} \cup \{0\}$,  defined on the set of all possible pairings  by
\begin{equation}
\mathds{1}_{\mathcal{G}, J ,m}(\underline{w}):=\left\{ \begin{array}{ll}  1 & \text{ if } \underline{w} \text{ is compatible with }   \mathcal{G} \text{ and  has exactly }  m  \text{ pairs  in }   J, \\0 & \text{ otherwise}. \end{array} \right. 
\end{equation}

\noindent
For every tuple $\underline{w}$ of $k$ pairs, 
\begin{equation}
\label{1G}
\mathds{1}_{\mathcal{G}}(\underline{w})=  \sum_{m=0}^{k} \mathds{1}_{\mathcal{G}, J,m}(\underline{w})
  \end{equation}
for all $\mathcal{G} \in \mathbb{F}_N$ and for all $J \subset \mathcal{V}(\mathcal{G})$. We plug (\ref{1G})  and (\ref{mu2})  into (\ref{DD13}) with $J= \textbf{I}_{i_0}$, and  we get that
\begin{equation}
\label{DD14}
\begin{split}
 \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O)=\sum_{k=0}^{\infty}  \sum_{m=0}^{k}  \underset{[0,t_N]^{2k}}{\int} d\mu_k (\underline{w})  \lambda( \underline{w})    \text{ } \mathds{1}_{\mathcal{G}, \textbf{I}_{i_0} ,m}(\underline{w}) \mathcal{T}_S \left[ \prod_{i=1}^{k}   \text{ }  {\bf{F}}(\underline{w})  \right] \left[ O_{t_N} \right].
\end{split}
\end{equation}
If  $\mathds{1}_{\mathcal{G}, \textbf{I}_{i_0} ,m}(\underline{w}) =1$ for some $m \in \mathbb{N}$, there are two unique  tuples $\underline{\tilde{w}}$ and $\underline{\hat{w}}$  with  $\underline{w}=\underline{\tilde{w}} \cup \underline{\hat{w}}$  such  that all times in $\underline{\hat{w}}$  lie in $\textbf{I}_{i_0}$ and  no time in   $\underline{\tilde{w}}$ lies in $\textbf{I}_{i_0}$. Up to a change of variables,  we can cut the integral in \eqref{DD14} into two distinct integrals. Exchanging the sum over $k$ with the sum over $m$, we  finally get that 
\begin{equation*}
%\label{DD16}
 \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O)=\sum_{k=0}^{\infty}  \underset{[0,t_N]^{2k}}{\int} d\mu_{k}  (\underline{\tilde{w}})  \lambda( \underline{\tilde{w}})  \text{ }  \mathds{1}_{\mathcal{G} \setminus \textbf{I}_{i_0} } ( \underline{\tilde{w}})\\
 \mathcal{T}_S \Big(    \textbf{F}( \underline{\tilde{w}})  \sum_{m=0}^{\infty}  \underset{ I_{i_0}}{\int} d\mu_m (\underline{\hat{w}})  \lambda( \underline{\hat{w}})    \mathcal{T}_S \left[   \textbf{F}( \underline{\hat{w}})  \right] \Big) \left[ O_{t_N} \right].
\end{equation*}
We recognize the operator $e^{i t_{i_{0}} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+1},t_{i_0}}e^{-i t_{i_0+1} \mathcal{L}_S}$  inside the parentheses; see \eqref{DD1'}.  Note that $\mathds{1}_{\mathcal{G} \setminus \textbf{I}_{i_0} } $  selects only the pairings compatible with $\mathcal{G}$ with no pairs in $\textbf{I}_{i_0}$. Repeating this procedure again for each isolated  interval,  we get the lemma.

\begin{lemma} 
\label{coiso}
Let $\mathcal{G} \in  \mathbb{F}_N$  with isolated  intervals $\textbf{I}_{i_0},...,\textbf{I}_{i_m}$, $i_0,...,i_m \neq N$. Then
\begin{equation}
\label{DDtt}
\begin{split}
 \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O) & =\sum_{k=0}^{\infty}      \underset{[0,t_N]^{2k}}{\int} d\mu_{k} (\underline{w})  \lambda( \underline{w})    \text{ }  \mathds{1}_{\mathcal{G} \setminus (\textbf{I}_{i_0}  \cup...\cup \textbf{I}_{i_m}) } (\underline{w}) \\
 &\mathcal{T}_S \left(      \textbf{F}( \underline{w} ) \text{ }  e^{i t_{i_{0}} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+1},t_{i_0}}e^{-i t_{i_0+1} \mathcal{L}_S}  \text{ } ... \text{ }e^{i t_{i_{m}} \mathcal{L}_S}\mathcal{Z}^{t_{i_m+1},t_{i_m}}e^{-i t_{i_m+1} \mathcal{L}_S} \right) \left[ O_{t_N} \right] 
 \end{split}
\end{equation}
for all $O \in \mathcal{B}(\mathcal{H}_S)$.
\end{lemma}
\vspace{2mm}

\subsection{Connected graphs and cluster expansion}
\label{secon}
\subsubsection{Construction of the set $\mathbb{G}_N$}
We use  that 
\begin{equation}
 \label{dec2}
 T_{t_i}= P_{t_i}+R_{t_i}
 \end{equation}
(see Lemma \ref{spectrum2})  to  rewrite $\langle \Psi(t_N)  \vert (O  \otimes 1)   \Psi(t_N) \rangle$  with a polymer expansion. Remark that
\begin{equation*}
e^{i t_{i_{0}} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+1},t_{i_0}}e^{-i t_{i_0+1} \mathcal{L}_S} e^{i t_{i_{0}+1} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+2},t_{i_0+1}} e^{-i t_{i_0+2} \mathcal{L}_S}
=e^{i t_{i_{0}} \mathcal{L}_S}\mathcal{Z}^{t_{i_0+1},t_{i_0}} \mathcal{Z}^{t_{i_0+2},t_{i_0+1}} e^{-i t_{i_0+2}  \mathcal{L}_S}
\end{equation*}
and that
\begin{equation*}
e^{i t_{N-1} \mathcal{L}_S} \mathcal{Z}^{t_{N},t_{N-1}} e^{-i t_{N} \mathcal{L}_S} O_{t_N}=e^{i t_{N-1} \mathcal{L}_S} \mathcal{Z}^{t_{N},t_{N-1}} O.
\end{equation*}
This shows that the operators $e^{it_j \mathcal{L}_S}$  cancel each other in the product inside the parentheses in \eqref{DDtt} if they are not located at the extremities of  a union of adjacent isolated  intervals. We   extend   the time ordering operator $\mathcal{T}_S$   in such a way that  $\mathcal{T}_S$ orders $e^{i t_{i_{l}} \mathcal{L}_S}$ on the right of $e^{-i t_{i_{l}} \mathcal{L}_S}$  and $e^{-i t_{i_{l}+1} \mathcal{L}_S}$ on the right of  $\mathcal{Z}^{t_{i_l+1},t_{i_l}}$. We   then rewrite
\begin{equation}
\label{DDt}
\begin{split}
 \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O)=\sum_{k=0}^{\infty} &    \underset{[0,t_N]^{2k} }{\int} d\mu_{k} (\underline{w})  \lambda( \underline{w})    \text{ }  \mathds{1}_{\mathcal{G} \setminus (\textbf{I}_{i_0}  \cup...\cup \textbf{I}_{i_m}) } (\underline{w}) \\
 &\mathcal{T}_S \Big(    \big( \prod_{l=0}^{m}  e^{-i t_{i_{l}+1} \mathcal{L}_S}  \big)    \textbf{F}( \underline{w} )   \big( \prod_{l=0}^{m}  e^{i t_{i_{l}} \mathcal{L}_S}  \big) \mathcal{Z}^{t_{i_0+1},t_{i_0}} \text{ } ... \text{ } \mathcal{Z}^{t_{i_m+1},t_{i_m}}  \Big) [ O_{t_N} ]
 \end{split}
\end{equation} 

\noindent We  construct a new set of graphs  by  inserting  (\ref{dec2}) into (\ref{DDt})  for each $\mathcal{G} \in \mathbb{F}_N$.  If $\mathcal{V}(\mathcal{G})$ contains  $m+1$ isolated intervals different from $I_{N+1}$, we get  $2^{m+1}$ terms of the form
\begin{equation}
\label{DDt2}
\begin{split}
\sum_{k=0}^{\infty}  &  \underset{[0,t_N]^{2k}  }{\int} d\mu_{k} (\underline{w})  \lambda( \underline{w})    \text{ }  \mathds{1}_{\mathcal{G} \setminus (\textbf{I}_{i_0}  \cup...\cup \textbf{I}_{i_m}) } (\underline{w}) \\
 &\mathcal{T}_S \Big(    \big( \prod_{l=0}^{m}  e^{-i t_{i_{l}+1} \mathcal{L}_S}  \big)    \textbf{F}( \underline{w} )   \big( \prod_{l=0}^{m}  e^{i t_{i_{l}} \mathcal{L}_S}  \big) P(t_{i_0}) R(t_{i_1})   ... \text{ } R(t_{i_m})   \Big) \left[ O_{t_N}  \right] .
 \end{split}
\end{equation}
We associate a graph to each of these $2^{m+1}$ terms. 
\vspace{2mm}

\noindent
\begin{construction} 
Let $\mathcal{G}$ be a graph in $\mathbb{F}_N$ with $m+1$ isolated vertices distinct from $\textbf{I}_N$. Using the decomposition \eqref{dec2}, we construct $2^{m+1}$ new graphs by following the procedure:
\begin{itemize}
\item If   $\textbf{I}_{i}$  carries a projection $P(t_{i})$, we erase $\textbf{I}_{i}$ from the vertex set of  $\mathcal{G}$.
\item If  $\textbf{I}_{i}$ carries  a perturbation $R(t_{i})$, we let $\textbf{I}_{i}$  in the vertex set of the graph, and mark it with the symbol
\begin{center}
\begin{tikzpicture}[scale=0.8]
\draw[ snake=zigzag]  (0.0,0.0) -- (2,0.0);
\fill (1,0) circle (0.1cm);
\end{tikzpicture}
\end{center}
\item  $\textbf{I}_{N}$ is  kept in the vertex set of the new graph and is marked  in bold.
\end{itemize}
We carry out  this construction for all  graphs in $\mathbb{F}_N$. We obtain a new finite set of graphs  that we denote by $\mathbb{G}_N$. A graph  $\mathcal{G}=(\mathcal{V}(\mathcal{G}),\mathcal{L}(\mathcal{G})) \in \mathbb{G}_N$ has a vertex set $\mathcal{V}(\mathcal{G})$ contained in $\lbrace \textbf{I}_0,..., \textbf{I}_{N} \rbrace$ and a set of lines   $\mathcal{L}(\mathcal{G})$. 
\end{construction}
\vspace{2mm}

\noindent As an example, it is easy to see that  we construct two new graphs from  the  figure \ref{bel2}.
\input{graph6}

  The vertex set $\mathcal{V}(\mathcal{G})$   of a graph $\mathcal{G}$ can be  divided into two disjoint subsets: the set of bound intervals, that we denote by $\mathcal{B}(\mathcal{G})$, and the set  of $R$-intervals (that carry a perturbation $R$), denoted by $\mathcal{R}(\mathcal{G})$.  A line $\mathscr{L}=(\textbf{I}_i,\textbf{I}_j) \in \mathcal{L}(\mathcal{G})$  $(i<j)$  binds  two intervals $\textbf{I}_i, \textbf{I}_j \in \mathcal{B}(\mathcal{G})$.  As in \eqref{DD12}, we  have that
 \begin{equation}
\label{DD12'}
 \mathcal{Z}^{t_N,0}(O)= \sum_{\mathcal{G} \in \mathbb{G}_N}  \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O),
 \end{equation}
but  the effective dynamics associated  to a graph $\mathcal{G} \in \mathbb{G}_N$ is now given by
\begin{equation}
\label{DDt2}
\begin{split}
 \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O): =\sum_{k=0}^{\infty}  &  \underset{[0,t_N]^{2k}  }{\int} d\mu_{k} (\underline{w})  \lambda( \underline{w})    \text{ }  \mathds{1}_{(\mathcal{B}(\mathcal{G}),\mathcal{L}(\mathcal{G})) } (\underline{w}) \\
 &\mathcal{T}_S \Big(    \big( \prod_{l,   \textbf{I}_l \notin \mathcal{B}(\mathcal{G})}  e^{-i t_{l+1} \mathcal{L}_S} e^{i t_{l} \mathcal{L}_S} \big)    \textbf{F}( \underline{w} )    \prod_{i, \textbf{I}_i \in \mathcal{R}(\mathcal{G})}   R(t_i)   \prod_{j, \textbf{I}_j \notin \mathcal{V}(\mathcal{G})}   P(t_j) \Big) [ \mathds{1}_S ],
 \end{split}
\end{equation}
where we have  set  $R(t_{N+1})=\textbf{L}(O)$.
We now decompose every  graph $\mathcal{G} \in \mathbb{G}_N$ into a disjoint union of connected subgraphs. The set of \textit{connected  graphs}  $\mathbb{G}^{c}_{N}$ is the polymer set of our cluster expansion. 
 
 \subsubsection{Construction of the set $\mathbb{G}_{N}^{c}$}
 A line $\mathscr{L} \in \mathcal{L}(\mathcal{G})$ is  represented by the drawing
\begin{center}
\begin{tikzpicture}[scale=0.5]

\fill (3.5,0) circle (0.1cm);
\fill (8.5,0) circle (0.1cm);


\draw[-] (3.5,0) -- (6, 1.0); 
\draw[-] (6,1) -- (8.5, 0.0);

\end{tikzpicture}
\end{center}
\noindent An \textit{adjacent edge} is an edge joining the center of two adjacent  intervals. There are 3 possible adjacent edges:
\begin{center}
\begin{tikzpicture}[scale=0.5]

\fill (3.5,0) circle (0.1cm);
\fill (6.5,0) circle (0.1cm);

\draw[-] (3.5,0) -- (6.5, 0.0); 

\fill (10.5,0) circle (0.1cm);
\fill (13.5,0) circle (0.1cm);
\draw[ -] (10.5,0) -- (12, 0.0); 
\draw[ snake=zigzag] (12,0) -- (13.5, 0.0); 


\fill (15.5,0) circle (0.1cm);
\fill (18.5,0) circle (0.1cm);
\draw[ snake=zigzag] (15.5,0) -- (17, 0.0); 
\draw[ -] (17,0) -- (18.5, 0.0); 

  
\end{tikzpicture}
\end{center}

A \textit{path}  from $\textbf{I}_{i}$ to $\textbf{I}_{j}$ is naturally defined as a non-broken succession of  lines and adjacent edges from the center of $\textbf{I}_i$ to the center of $\textbf{I}_j$; see the figure below. We say that a graph $\mathcal{G} \in \mathbb{G}_{N}$ is \textit{connected} if  there is a path joining  $\textbf{I}_i$ to  $\textbf{I}_j$ for all  $\textbf{I}_i \neq \textbf{I}_j \in \mathcal{V}(\mathcal{G})$. The set of \textit{connected graphs} is denoted by $\mathbb{G}^{c}_{N}$.
 \begin{center}
\begin{tikzpicture}[scale=0.5]

\fill (3.5,0) circle (0.1cm);
\fill (6.5,0) circle (0.1cm);
\fill (-1,0) circle (0.1cm);

 \draw (-1,0) node[below] {$\textbf{I}_{t_1}$};
  \draw (12.5,0) node[below] {$\textbf{I}_{t_2}$};
  
\draw[-] (6.5,0) -- (9.5, 0.0); 
\draw[-] (3.5,0) -- (5, 1.0); 
\draw[-] (5,1.0) -- (6.5, 0.0); 

\fill (9.5,0) circle (0.1cm);
\fill (12.5,0) circle (0.1cm);
\draw[ snake=zigzag] (10.5,0) -- (12.5, 0.0); 
\draw[ -] (9.5,0) -- (10.5, 0.0); 

\draw[ -] (-1,0) -- (1.25, 1.0); 
\draw[ -] (1.25, 1.0) -- (3.5, 0.0); 

 \draw (6.5,-1.5) node[below] {\footnotesize A path from $\textbf{I}_{t_1}$ to  $\textbf{I}_{t_2}$};

\end{tikzpicture}
\end{center}
\input{graph7}
\vspace{2mm}

It is  useful to introduce the notion of \textit{maximal union of adjacent vertices }.  We say that a disjoint union   $U=\cup_i  \text{ } \textbf{I}_{i} \subset \mathcal{V}(\mathcal{G})$ of  adjacent  vertices  is  a maximal union of adjacent vertices  if,  for any $\textbf{I}_{i}, \textbf{I}_{j} \in U$,  there is an adjacent path joining $\textbf{I}_{i}$ to $\textbf{I}_{j}$,  and if $U$ is the biggest set in $\mathcal{V}(\mathcal{G})$ in the sense of the inclusion having this property.  We denote by  $\mathcal{U}(\mathcal{G})$ the set of maximal unions of adjacent vertices  of  $\mathcal{G}$.  Maximal unions of adjacent vertices are  surrounded at their  extremities by  one-dimensional projections $P$, and this is the reason why we  need them to write the polymer expansion.  


\subsubsection{The polymer expansion}
Before writing our polymer expansion for the effective dynamics $\mathcal{Z}^{t_N,0}$, we introduce three further useful notations. We define
\begin{align}
\label{mmm}
m(A)&:= \min \{ i \mid  \textbf{I}_{i} \in A \}-1,\\
\label{MMM}
M(A)&:=\max \{ i \mid  \textbf{I}_{i} \in A \}+1
\end{align}
for all sets $A \subset \mathcal{V}(\mathcal{G})$ and 
\begin{equation}
\mbox{dist} \left(\mathcal{G}, \mathcal{G}' \right)=\underset{\textbf{I}_{i} \in \mathcal{V}(\mathcal{G}), \text{ } \textbf{I}_{j} \in \mathcal{V}(\mathcal{G'})}{\min}  (\vert i-j  \vert-1) 
\end{equation}
for all  $\mathcal{G}$, $\mathcal{G'} \in   \mathbb{G}_N$. Two  adjacent graphs have a distance equal to $0$. It is clear that any graph $\mathcal{G} \in \mathbb{G}_N$ possesses a unique decomposition into connected subgraphs, separated each other by a distance bigger or equal to one.  This remarks leads to the lemma


\begin{lemma}
\label{facto}
Let $\mathcal{G} =\mathcal{G}_1 \vee ... \vee \mathcal{G}_q  \in \mathbb{G}_N$, with $\mathcal{G}_1,...,\mathcal{G}_q \in  \mathbb{G}^{c}_{N}$  and $ \text{dist}(\mathcal{G}_i,\mathcal{G}_j) \geq 1$ for all $ i\neq j$.  Then
\begin{equation}
\label{prodd}
\langle \varphi  \vert \mathcal{Z}_{\mathcal{G}}^{t_N,0}(O)  \varphi \rangle  =p(\mathcal{G}_1)\text{ }... \text{ }p(\mathcal{G}_q)
\end{equation}

\noindent where $p: \mathbb{G}_{N}^{c} \rightarrow \mathbb{C}$ is  defined by
\begin{equation}
\label{p(G)}
p(\mathcal{G}):=\sum_{k=0}^{\infty }  \underset{[0,t_N]^{2k}} {\int} d\mu_k  (\underline{w})  \lambda( \underline{w})    \text{ }   \mathds{1}_{(\mathcal{B}(\mathcal{G}),\mathcal{L}(\mathcal{G})) } (\underline{w})  \text{ F}(\underline{w})   \prod_{U \in \mathcal{U}(\mathcal{G})} h(U,\underline{w})
\end{equation}
and where we have set
\begin{equation*}
 h(U ,\underline{w}):=\langle \Pi (t_{m(U)}) \vert \mathcal{T}_S \Big( \underset{i, \textbf{I}_i \in U \cap \mathcal{B}(\mathcal{G}) }{\prod} \Big[ e^{-it_{i} \mathcal{L}_S} \big( \prod_{(t,r) \in  \underline{w} \cap \textbf{I}_i } (i G)(t,r) \big) e^{it_{i+1} \mathcal{L}_S} \Big]   \underset{j, \textbf{I}_j \in U \cap \mathcal{R}(\mathcal{G}) }{\prod} R(t_j) \Big) 1_S \rangle,
\end{equation*}
\begin{equation*}
\Pi(t_{-1}):= \vert \varphi  \rangle \langle \varphi \vert  \qquad   \text{ and } \qquad  R(t_{N}):=\textbf{L}(O).
\end{equation*}
 \end{lemma}
\vspace{2mm}

\noindent  The proof of Lemma \ref{facto} is carried out in the appendix.   Lemma \ref{facto}  readily  implies   that the  expectation value $\langle \Psi(t_N) \vert  O    \Psi(t_N) \rangle$ can be rewritten as a cluster expansion over the polymer set $\mathbb{G}^{c}_{N}$.



\begin{proposition}
\label{clustt}
\begin{align}
\label{eqclu1}
\langle \Psi (t_N) \vert (O  \otimes 1)   \Psi(t_N) \rangle&=  \sum_{q=1}^{N} \frac{1}{q!} \underset{\text{dist}(\mathcal{G}_i,\mathcal{G}_j) \geq 1, \text{ } \exists i_0, \text{ }\textbf{I}_{N} \in \mathcal{V}( \mathcal{G}_{i_0})}{\underset{\mathcal{G}_1,...,\mathcal{G}_q \in \mathbb{G}^{c}_{N}}{\sum}}   p\left(\mathcal{G}_1\right)...\text{ }p\left(\mathcal{G}_q\right), \\
\label{eqclu2}
\langle   \Psi (t_N) \vert   \Psi (t_N) \rangle&=   1 +  \sum_{q=1}^{N} \frac{1}{q!} \underset{\text{dist}(\mathcal{G}_i,\mathcal{G}_j) \geq 1,  \text{ }\textbf{I}_{N} \notin \mathcal{V}( \mathcal{G}_{i}) } {\underset{\mathcal{G}_1,...,\mathcal{G}_q \in \mathbb{G}^{c}_{N}}{\sum}}   \text{ } \text{ } p\left(\mathcal{G}_1\right)...\text{ }p\left(\mathcal{G}_q\right).
\end{align}
\end{proposition}
\vspace{4mm}


\begin{remark}The factor $q!$ comes from the permutation of the graphs  in $\mathbb{G}^{c}_{N}$ . The sum over $q$  is finite and ends  if  it is  not possible to find  $\mathcal{G}_1,...,\mathcal{G}_q \in \mathbb{G}^{c}_{N}$ such that  $\mathcal{G} =\mathcal{G}_1 \vee ... \vee \mathcal{G}_m  \in \mathbb{G}_N$, with $\mathcal{G}_1,...,\mathcal{G}_m \in  \mathbb{G}^{c}_{N}$  and $ \text{dist}(\mathcal{G}_i,\mathcal{G}_j) \geq 1$ for all $ i\neq j$.
\end{remark}
















